Measurement of the CKM angle $\gamma$ from a combination of LHCb results

A combination of measurements sensitive to the CKM angle $\gamma$ from LHCb is performed. The inputs are from analyses of time-integrated $B^{+}\rightarrow DK^+$, $B^{0} \rightarrow D K^{*0}$, $B^{0} \rightarrow D K^+ \pi^-$ and $B^{+} \rightarrow D K^+\pi^+\pi^-$ tree-level decays. In addition, results from a time-dependent analysis of $B_{s}^{0} \rightarrow D_{s}^{\mp}K^{\pm}$ decays are included. The combination yields $\gamma = (72.2^{+6.8}_{-7.3})^\circ$, where the uncertainty includes systematic effects. The 95.5% confidence level interval is determined to be $\gamma \in [55.9,85.2]^\circ$. A second combination is investigated, also including measurements from $B^{+} \rightarrow D \pi^+$ and $B^{+} \rightarrow D \pi^+\pi^-\pi^+$ decays, which yields compatible results.

==> LHCb_Authorship_flat_arXiv_12-Jul-2016.tex <==
LHCb collaboration: 
R. Aaij,
B. Adeva,
M. Adinolfi,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
S. Ali,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
R.B. Appleby,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
E. Aslanides,
G. Auriemma,
M. Baalouch,
I. Babuschkin,
S. Bachmann,
J.J. Back,
A. Badalov,
C. Baesso,
S. Baker,
W. Baldini,
R.J. Barlow,
C. Barschel,
S. Barsuk,
W. Barter,
M. Baszczyk,
V. Batozskaya,
B. Batsukh,
V. Battista,
A. Bay,
L. Beaucourt,
J. Beddow,
F. Bedeschi,
I. Bediaga,
L.J. Bel,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
J. Benton,
A. Berezhnoy,
R. Bernet,
A. Bertolin,
F. Betti,
M.-O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bifani,
P. Billoir,
T. Bird,
A. Birnkraut,
A. Bitadze,
A. Bizzeti,
T. Blake,
F. Blanc,
J. Blouw,
S. Blusk,
V. Bocci,
T. Boettcher,
A. Bondar,
N. Bondar,
W. Bonivento,
A. Borgheresi,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
E. Bowen,
C. Bozzi,
S. Braun,
M. Britsch,
T. Britton,
J. Brodzicka,
E. Buchanan,
C. Burr,
A. Bursche,
J. Buytaert,
S. Cadeddu,
R. Calabrese,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D. Campora Perez,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carson,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
L. Castillo Garcia,
M. Cattaneo,
Ch. Cauet,
G. Cavallero,
R. Cenci,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
S. Chen,
S.-F. Cheung,
V. Chobanova,
M. Chrzaszcz,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
V. Coco,
J. Cogan,
E. Cogneras,
V. Cogoni,
L. Cojocariu,
G. Collazuol,
P. Collins,
A. Comerma-Montells,
A. Contu,
A. Cook,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
S. Cunliffe,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
E. Dall'Occo,
J. Dalseno,
P.N.Y. David,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.-T. Dean,
D. Decamp,
M. Deckenhoff,
L. Del Buono,
M. Demmer,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
K. Dungs,
P. Durante,
R. Dzhelyadin,
A. Dziurda,
A. Dzyuba,
N. D{\'e}l{\'e}age,
S. Easo,
M. Ebert,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
Ch. Elsasser,
S. Ely,
S. Esen,
H.M. Evans,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
R. Fay,
D. Fazzini,
D. Ferguson,
V. Fernandez Albor,
A. Fernandez Prieto,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiore,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
K. Fohl,
M. Fontana,
F. Fontanelli,
D.C. Forshaw,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
E. Furfaro,
C. F{\"a}rber,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
P.J. Garsed,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Ph. Ghez,
S. Gian{\`\i},
V. Gibson,
O.G. Girard,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
M. Grabalosa G{\'a}ndara,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
P. Griffith,
L. Grillo,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
E. Gushchin,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
S. Hall,
B. Hamilton,
X. Han,
S. Hansmann-Menzemer,
N. Harnew,
S.T. Harnew,
J. Harrison,
M. Hatch,
J. He,
T. Head,
A. Heister,
K. Hennessy,
P. Henrard,
L. Henry,
J.A. Hernando Morata,
E. van Herwijnen,
M. He{\ss},
A. Hicheur,
D. Hill,
C. Hombach,
H. Hopchev,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
N. Hussain,
D. Hutchcroft,
M. Idzik,
P. Ilten,
R. Jacobsson,
A. Jaeger,
J. Jalocha,
E. Jans,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
W. Kanso,
M. Karacson,
J.M. Kariuki,
S. Karodia,
M. Kecke,
M. Kelsey,
I.R. Kenyon,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
T. Kirn,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
M. Kolpin,
I. Komarov,
R.F. Koopman,
P. Koppenburg,
A. Kosmyntseva,
A. Kozachuk,
M. Kozeiha,
L. Kravchuk,
K. Kreplin,
M. Kreps,
P. Krokovny,
F. Kruse,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
K. Kurek,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
D. Lambert,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
J. van Leerdam,
J.-P. Lees,
A. Leflat,
J. Lefran{\c{c}}ois,
R. Lef{\`e}vre,
F. Lemaitre,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
Y. Li,
T. Likhomanenko,
R. Lindner,
C. Linn,
F. Lionetto,
B. Liu,
X. Liu,
D. Loh,
I. Longstaff,
J.H. Lopes,
D. Lucchesi,
M. Lucio Martinez,
H. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
O. Maev,
K. Maguire,
S. Malde,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
P. Manning,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
P. Marino,
J. Marks,
G. Martellotti,
M. Martin,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
D. Martins Tostes,
L.M. Massacrier,
A. Massafferri,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
B. Maurin,
A. Mazurov,
M. McCann,
J. McCarthy,
A. McNab,
R. McNulty,
B. Meadows,
F. Meier,
M. Meissner,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
M.-N. Minard,
D.S. Mitzel,
A. Mogini,
J. Molina Rodriguez,
I.A. Monroy,
S. Monteil,
M. Morandin,
P. Morawski,
A. Mord{\`a},
M.J. Morello,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mulder,
M. Mussini,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
M. Neuner,
A.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
T. Nikodem,
A. Novoselov,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
J.M. Otalora Goicochea,
A. Otto,
P. Owen,
A. Oyanguren,
P.R. Pais,
A. Palano,
F. Palombo,
M. Palutan,
J. Panman,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
G.D. Patel,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
M. Petruzzo,
E. Picatoste Olloqui,
B. Pietrzyk,
M. Pikies,
D. Pinci,
A. Pistone,
A. Piucci,
S. Playfer,
M. Plo Casasus,
T. Poikela,
F. Polci,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
A. Popov,
D. Popov,
B. Popovici,
S. Poslavskii,
C. Potterat,
E. Price,
J.D. Price,
J. Prisciandaro,
A. Pritchard,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
G. Punzi,
W. Qian,
R. Quagliani,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
I. Raniuk,
G. Raven,
F. Redi,
S. Reichert,
A.C. dos Reis,
C. Remon Alepuz,
V. Renaudin,
S. Ricciardi,
S. Richards,
M. Rihl,
K. Rinnert,
V. Rives Molina,
P. Robbe,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
P. Rodriguez Perez,
A. Rogozhnikov,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
J.W. Ronayne,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
P. Ruiz Valls,
J.J. Saborido Silva,
E. Sadykhov,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
A. Sarti,
C. Satriano,
A. Satta,
D.M. Saunders,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schlupp,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
K. Schubert,
M. Schubiger,
M.-H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
P. Seyfert,
M. Shapkin,
I. Shapoval,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
A. Shires,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
M. Sirendi,
N. Skidmore,
T. Skwarnicki,
E. Smith,
I.T. Smith,
J. Smith,
M. Smith,
H. Snoek,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
P. Spradlin,
S. Sridharan,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
S. Stevenson,
S. Stoica,
S. Stone,
B. Storaci,
S. Stracka,
M. Straticiuc,
U. Straumann,
L. Sun,
W. Sutcliffe,
K. Swientek,
V. Syropoulos,
M. Szczekowski,
T. Szumlak,
S. T'Jampens,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
S. Topp-Joergensen,
F. Toriello,
E. Tournefier,
S. Tourneur,
K. Trabelsi,
M. Traill,
M.T. Tran,
M. Tresch,
A. Trisovic,
A. Tsaregorodtsev,
P. Tsopelas,
A. Tully,
N. Tuning,
A. Ukleja,
A. Ustyuzhanin,
U. Uwer,
C. Vacca,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
A. Vallier,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
M. Vernet,
M. Vesterinen,
B. Viaud,
D.  Vieira,
M. Vieites Diaz,
X. Vilasis-Cardona,
V. Volkov,
A. Vollhardt,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
C. Vo{\ss},
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
C. Wallace,
R. Wallace,
J. Walsh,
J. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
M. Whitehead,
J. Wicht,
G. Wilkinson,
M. Wilkinson,
M. Williams,
M.P. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
J. Wimberley,
J. Wishahi,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wraight,
S. Wright,
K. Wyllie,
Y. Xie,
Z. Xing,
Z. Xu,
Z. Yang,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
L. Zhang,
Y. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
A. Zhokhov,
X. Zhu,
V. Zhukov,
S. Zucchelli

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}


==> app_correlations.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section*{Appendix: Correlation matrices of input measurements}
\label{sec:correlationsofinputs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \Dzhh GLW/ADS correlations.}
\label{tab:glwadshhCor}
  \input{glwads-dk-hh_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \Dzhh GLW/ADS correlations.}
\label{tab:glwadshhCorSyst}
  \input{glwads-dk-hh_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \Dzhpipipi GLW/ADS-like correlations.}
\label{tab:glwadsk3piCor}
  \input{glwads-dk-hpipipi_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \Dzhpipipi GLW/ADS-like correlations.}
\label{tab:glwadsk3piCorSyst}
  \input{glwads-dk-hpipipi_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \Dzhhpiz GLW/ADS-like correlations.}
\label{tab:glwadshhpizCor}
  \input{glwads-dk-hhpiz_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \Dzhhpiz GLW/ADS-like correlations.}
\label{tab:glwadshhpizCorSyst}
  \input{glwads-dk-hhpiz_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \DzKShh GGSZ correlations.}
\label{tab:ggszCor}
  \input{ggsz-dk_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \DzKShh GGSZ correlations.}
\label{tab:ggszCorSyst}
  \input{ggsz-dk_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \DKSKpi GLS correlations.}
\label{tab:glsCor}
  \input{gls_stat}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \DKSKpi GLS correlations.}
\label{tab:glsCorSyst}
  \input{gls_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \BdDzKstz ADS correlations.}
\label{tab:glwadsdkstCor}
  \input{ads-dkstz_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \BdDzKstz ADS correlations.}
\label{tab:glwadsdkstCorSyst}
  \input{ads-dkstz_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \BdDzKpi GLW-Dalitz correlations.}
\label{tab:glwkstCor}
  \input{glw-dalitz-dkstz_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \BdDzKpi GLW-Dalitz correlations.}
\label{tab:glwkstCorSyst}
  \input{glw-dalitz-dkstz_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \BdDzKstz GGSZ correlations.}
\label{tab:ggszkstCor}
  \input{ggsz-dkstz_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \BdDzKstz GGSZ correlations.}
\label{tab:ggszkstCorSyst}
  \input{ggsz-dkstz_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \BuDKpipi GLW/ADS-like correlations.}
\label{tab:glwadsdkpipiCor}
  \input{glwads-dkpipi-hh_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \BuDKpipi GLW/ADS-like correlations.}
\label{tab:glwadsdkpipiCorSyst}
  \input{glwads-dkpipi-hh_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!hbtp]
\small
\centering
\caption{Statistical \BsDsK correlations.}
\label{tab:dskCor}
  \input{dsk_stat}
\end{table}

\begin{table}[!hbtp]
\small
\centering
\caption{Systematic \BsDsK correlations.}
\label{tab:dskCorSyst}
  \input{dsk_syst}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!hbtp]
\small
\centering
\caption{Correlations of the \DzKpipipi and \DzKpipiz parameters from CLEO and LHCb.}
\label{tab:cleoCor}
  \input{cleo_stat}
\end{table}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table}[!hbtp]
\small
\centering
\caption{Correlations of the HFAG charm parameters (CHARM 2015, ``Fit 3'', \CP violation allowed).}
\label{tab:hfagCor}
  \input{hfag_stat}
\end{table}

\clearpage


==> cds_titleabstract.tex <==

Improved constraints on $\gamma$ from $B^\pm\to DK^\pm$ decays
including first results on 2012 data


Preliminary results for the CKM angle $\gamma$ are presented, from
a combination of measurements using $B^\pm\to DK^\pm$ decays,
where $D$ denotes an admixture of $D^0$ and $\overline{D}^0$ mesons.
Results for the $D$ final states $K^+K^-$, $\pi^+\pi^-$, $K^\pm \pi^\mp$,
and $K^\pm \pi^\mp \pi^\pm \pi^\mp$
are based on a dataset corresponding to $1\,{\rm fb}^-1$ of integrated
luminosity recorded at $\sqrt{s}=7\,{\rm TeV}$ in 2011.
Results for the $D$ decays into $K_S\pi^+\pi^-$ and $K_S K^+K^-$
are based on a dataset corresponding to $3\,{\rm fb}^-1$ recorded at 
$\sqrt{s}=7$ and $8\,{\rm TeV}$ in 2011 and 2012, respectively.
A best fit value of $\gamma = 67.2^\circ$ is found, and
confidence intervals are set:
\begin{align*}
\gamma \in [55.1, 79.1]^\circ &~{\rm at~68\%~CL}\,,\\
\gamma \in [43.9, 89.5]^\circ &~{\rm at~95\%~CL}\,,
\end{align*}
where the first interval is translated into $\gamma = (67 \pm 12)^\circ$
at 68\% CL, and all quoted values are modulo $180^\circ$.


==> cleo_syst.tex <==
\begin{tabular}{ l |cccccc}
\hline
                & \kdKppp & \ddKppp & \kdKpp & \ddKpp & \rdKppp & \rdKpp\\
\hline
\kdKppp         &       1 &       0 &       0 &       0 &       0 &       0  \\
\ddKppp         &       0 &       1 &       0 &       0 &       0 &       0  \\
\kdKpp          &       0 &       0 &       1 &       0 &       0 &       0  \\
\ddKpp          &       0 &       0 &       0 &       1 &       0 &       0  \\
\rdKppp         &       0 &       0 &       0 &       0 &       1 &       0  \\
\rdKpp          &       0 &       0 &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> detector.tex <==
\section{Detector and simulation}
\label{sec:Detector}
The paragraph below can be used for the detector
description. Modifications may be required in specific papers to fit
within page limits, to enhance particular detector elements or to
introduce acronyms used later in the text. For journals where strict
word counts are applied (for example, PRL), and space is at a premium,
it may be sufficient to write, as a minimum: ``The LHCb detector is a 
single-arm forward spectrometer covering the pseudorapidity range 
$2 < \eta < 5$, 
described in detail in Refs.~\cite{Alves:2008zz,LHCb-DP-2014-002}''. 
A slightly longer version could specify the most relevant sub-detectors, {\it e.g} 
``The LHCb 
detector~\cite{Alves:2008zz,LHCb-DP-2014-002} is a
single-arm forward spectrometer covering the pseudorapidity range $2 < \eta < 5$, designed for
the study of particles containing b or c quarks. The detector elements that are particularly
relevant to this analysis are: a silicon-strip vertex detector surrounding the pp interaction
region that allows c- and b-hadrons to be identified from their characteristically long
flight distance; a tracking system that provides a measurement of momentum, $p$, of charged
particles; and two ring-imaging Cherenkov detectors that are able to discriminate between
different species of charged hadrons.'' 

\begin{verbatim}
In the following paragraph, references to the individual detector 
performance papers are marked with a * and should only be included 
if the analysis relies on numbers or methods described in the specific 
papers. Otherwise, a reference to the overall detector performance 
paper~\cite{LHCb-DP-2014-002} will suffice. Note also that the text 
defines the acronyms for primary vertex, PV, and impact parameter, IP. 
Remove either of those in case it is not used later on.
\end{verbatim}

The \lhcb detector~\cite{Alves:2008zz,LHCb-DP-2014-002} is a single-arm forward
spectrometer covering the \mbox{pseudorapidity} range $2<\eta <5$,
designed for the study of particles containing \bquark or \cquark
quarks. The detector includes a high-precision tracking system
consisting of a silicon-strip vertex detector surrounding the $pp$
interaction region~\cite{LHCb-DP-2014-001}\verb!*!, a large-area silicon-strip detector located
upstream of a dipole magnet with a bending power of about
$4{\mathrm{\,Tm}}$, and three stations of silicon-strip detectors and straw
drift tubes~\cite{LHCb-DP-2013-003}\verb!*! placed downstream of the magnet.
The tracking system provides a measurement of momentum, \ptot, of charged particles with
a relative uncertainty that varies from 0.5\% at low momentum to 1.0\% at 200\gevc.
The minimum distance of a track to a primary vertex (PV), the impact parameter (IP), 
is measured with a resolution of $(15+29/\pt)\mum$,
where \pt is the component of the momentum transverse to the beam, in\,\gevc.
Different types of charged hadrons are distinguished using information
from two ring-imaging Cherenkov detectors~\cite{LHCb-DP-2012-003}\verb!*!. 
Photons, electrons and hadrons are identified by a calorimeter system consisting of
scintillating-pad and preshower detectors, an electromagnetic
calorimeter and a hadronic calorimeter. Muons are identified by a
system composed of alternating layers of iron and multiwire
proportional chambers~\cite{LHCb-DP-2012-002}\verb!*!.
The online event selection is performed by a trigger~\cite{LHCb-DP-2012-004}\verb!*!, 
which consists of a hardware stage, based on information from the calorimeter and muon
systems, followed by a software stage, which applies a full event
reconstruction.

A more detailed description of the 'full event reconstruction' could be:
\begin{itemize}
\item The trigger~\cite{LHCb-DP-2012-004}\verb!*! consists of a
hardware stage, based on information from the calorimeter and muon
systems, followed by a software stage, in which all charged particles
with $\pt>500\,(300)\mev$ are reconstructed for 2011\,(2012) data.
For triggers that require neutral particles, 
energy deposits in the electromagnetic calorimeter are 
analysed to reconstruct \piz and $\gamma$ candidates.
\end{itemize}

The trigger description has to be specific for the analysis in
question. In general, you should not attempt to describe the full
trigger system. Below are a few variations that inspiration can be
taken from. First from a hadronic analysis, and second from an
analysis with muons in the final state. In case you have to look 
up specifics of a certain trigger, a detailed description of the trigger 
conditions for Run 1 is available in Ref.~\cite{LHCb-PUB-2014-046}. 
{\bf Never cite this note in a PAPER or CONF-note.} 


\begin{itemize}
\item At the hardware trigger stage, events are required to have a muon with high \pt or a
  hadron, photon or electron with high transverse energy in the calorimeters. For hadrons,
  the transverse energy threshold is 3.5\gev.
  The software trigger requires a two-, three- or four-track
  secondary vertex with a significant displacement from the primary
  $pp$ interaction vertices. At least one charged particle
  must have a transverse momentum $\pt > 1.7\gevc$ and be
  inconsistent with originating from a PV.
  A multivariate algorithm~\cite{BBDT} is used for
  the identification of secondary vertices consistent with the decay
  of a \bquark hadron.
%\item The software trigger requires a two-, three- or four-track
%  secondary vertex with a large sum of the transverse momentum, \pt, of
%  the tracks and a significant displacement from the primary $pp$
%  interaction vertices~(PVs). At least one track should have $\pt >
%  1.7\gevc$ and \chisqip with respect to any
%  primary interaction greater than 16, where \chisqip is defined as the
%  difference in \chisq of a given PV reconstructed with and
%  without the considered track.\footnote{If this sentence is used to define \chisqip
%  for a composite particle instead of for a single track, replace ``track'' by ``particle'' or ``candidate''}
% A multivariate algorithm~\cite{BBDT} is used for
%  the identification of secondary vertices consistent with the decay
%  of a \bquark hadron.
\item The $\decay{\Bd}{\Kstarz\mumu}$ signal candidates are first required
      to pass the hardware trigger, which selects events containing at least
      one muon with transverse momentum $\pt>1.48\gevc$ in the 7\tev data or
      $\pt>1.76\gevc$ in the 8\tev data.  In the subsequent software
      trigger, at least one of the final-state particles is required to 
      have $\pt>1.7\gevc$ in the 7\tev data or $\pt>1.6\gevc$ in the 8\tev 
      data, unless the particle is identified as a muon in which case 
      $\pt>1.0\gevc$ is required. The final-state particles that 
      satisfy these transverse momentum criteria are also required 
      to have an impact parameter larger than $100\mum$ with respect 
      to all PVs in the event. Finally, the tracks of two or more of 
      the final-state particles are required to form a vertex that is 
      significantly displaced from the PVs." 

%  Candidate events are first required to pass the hardware trigger,
%  which selects muons with a transverse momentum $\pt>1.48\gevc$ 
%  in the 7\tev data or $\pt>1.76\gevc$ in the 8\tev data.
%  In the subsequent software trigger, at least
%  one of the final-state particles is required to have both
%  $\pt>0.8\gevc$ and impact parameter larger than $100\mum$ with respect to all
%  of the primary $pp$ interaction vertices~(PVs) in the
%  event. Finally, the tracks of two or more of the final-state
%  particles are required to form a vertex that is significantly
%  displaced from the PVs.
\end{itemize}

An example to describe the use of both TOS and TIS events:
\begin{itemize}
\item In the offline selection, trigger signals are associated with reconstructed particles.
%Selection requirements can therefore be made not only on the trigger requirement,
%but on whether the decision was due to the signal candidate, other particles produced in the $pp$ collision, or a combination of both.
Selection requirements can therefore be made on the trigger selection itself
and on whether the decision was due to the signal candidate, other particles produced in the $pp$ collision, or a combination of both.
\end{itemize}

A good example of a description of long and downstream \KS is given in 
Ref.~\cite{LHCb-PAPER-2014-006}:
\begin{itemize}
\item
Decays of \decay{\KS}{\pip\pim} are reconstructed in two different categories:
the first involving \KS mesons that decay early enough for the
daughter pions to be reconstructed in the vertex detector; and the
second containing \KS that decay later such that track segments of the
pions cannot be formed in the vertex detector. These categories are
referred to as \emph{long} and \emph{downstream}, respectively. The
long category has better mass, momentum and vertex resolution than the
downstream category.
\end{itemize}

The description of our software stack for simulation is often
causing trouble. The following paragraph can act as inspiration but
with variations according to the level of detail required and if
mentioning of \eg \photos is required.
\begin{itemize}
\item In the simulation, $pp$ collisions are generated using
\pythia~\cite{Sjostrand:2006za,*Sjostrand:2007gs} 
(In case only \pythia 6 is used, remove \verb=*Sjostrand:2007gs= from this citation; if 
only \pythia 8 is used, then reverse the order of the papers in the citation.)
 with a specific \lhcb
configuration~\cite{LHCb-PROC-2010-056}.  Decays of hadronic particles
are described by \evtgen~\cite{Lange:2001uf}, in which final-state
radiation is generated using \photos~\cite{Golonka:2005pn}. The
interaction of the generated particles with the detector, and its response,
are implemented using the \geant
toolkit~\cite{Allison:2006ve, *Agostinelli:2002hh} as described in
Ref.~\cite{LHCb-PROC-2011-006}.
\end{itemize}

Many analyses depend on boosted decision trees. It is inappropriate to
use TMVA as the reference as that is merely an implementation of the
BDT algorithm. Rather it is suggested to write

In this paper we use a boosted decision tree~(BDT)~\cite{Breiman,AdaBoost} to
separate signal from background.

When describing the integrated luminosity of the data set, do not use
expressions like ``1.0\,fb$^{-1}$ of data'', but \eg 
``data corresponding to an integrated luminosity of 1.0\,fb$^{-1}$'', 
or ``data obtained from 3\,fb$^{-1}$ of integrated luminosity''. 

For analyses where the periodical reversal of the magnetic field is crucial, 
\eg in measurements of direct \CP violation, the following description can be
used as an example phrase: 
``The polarity of the dipole magnet is reversed periodically throughout data-taking.
The configuration with the magnetic field vertically upwards, \MagUp (downwards, \MagDown), bends positively (negatively)
charged particles in the horizontal plane towards the centre of the LHC.''
Only use the \MagUp, \MagDown symbols if they are used extensively in tables or figures.


==> figures.tex <==
% $Id: figures.tex 61168 2014-09-25 23:10:50Z roldeman $
% ===============================================================================
% Purpose: including figures in the standard template
% Author: Tomasz Skwarnicki, Ulrik Egede
% Created on: 2010-09-24
% ===============================================================================

\section{Figures}
\label{sec:Figures}

A standard \lhcb style file for use in production of figures in \root
is in the \urania package \texttt{RootTools/LHCbStyle} or directly in
\svn at
\texttt{svn+ssh://svn.cern.ch/reps/lhcb/Urania/trunk/RootTools/LHCbStyle}. It
is not mandatory to use this style, but it makes it easier to follow
the recommendations below.

Figure~\ref{fig:example} shows an example of how to include an eps
or pdf figure with the \texttt{\textbackslash includegraphics} command
(eps figures will not work with \texttt{pdflatex}). Note that if the
graphics sits in \texttt{figs/myfig.pdf}, you can just write
\texttt{\textbackslash includegraphics\{myfig\}} as the \texttt{figs}
subdirectory is searched automatically and the extension \texttt{.pdf}
(\texttt{.eps}) is automatically added for \texttt{pdflatex}
(\texttt{latex}).
\begin{figure}[tb]
  \begin{center}
    \includegraphics[width=0.49\linewidth]{Example1DPlot-python-1}\put(-32,133){(a)}
    \includegraphics[width=0.49\linewidth]{Example1DPlot-python-1_sim}\put(-32,133){(b)}
    \vspace*{-1.0cm}
  \end{center}
  \caption{
    %\small %captions should be a little bit smaller than main text
    Example plots for (a) data and (b) simulation using the \lhcb style from the \urania package
    \texttt{RootTools/LHCbStyle}. The signal data is shown as points
    with the signal component as yellow (light shaded), background 1 as green
    (medium shaded) and background 2 as blue (dark shaded).}
  \label{fig:example}
\end{figure}

\begin{enumerate}

\item Figures should be legible at the size they will appear in the
  publication, with suitable line width.  Their axes should be
  labelled, and have suitable units (e.g. avoid a mass plot with
  labels in \mevcc if the region of interest covers a few \gevcc
  and all the numbers then run together).  Spurious background shading
  and boxes around text should be avoided.

\item For the $y$-axis, ``Entries'' or ``Candidates'' is approriate in case no
background subtraction has been applied. Otherwise ``Yield'' or ``Decays''
may be more appropriate. If the unit on the $y$-axis corresponds to 
the yield per bin, indicate so, for example ``Entries / ( 5\mevcc )'' or ``Entries per 5\mevcc''.


\item Fit curves should not obscure the data points, and
   data points are best (re)drawn over the fit curves.

\item Colour may be used in figures, but the distinction between
  differently coloured areas or lines should be clear also when the
  document is printed in black and white, for example through
  differently dashed lines. The \lhcb style mentioned above implements
  a colour scheme that works well but individual adjustments might be
  required.

\item Using different hatching styles helps to disinguished filled areas, 
also in black and white prints. Hatching styles 3001-3025 should be
avoided since they behave unpredictably under zooming and scaling. 
Good styles for ``falling hatched'' and ``rising hatched'' are 3345 and 3354.


\item Figures with more than one part should have the parts labelled
  (a), (b) \etc, with a corresponding description in the caption;
  alternatively they should be clearly referred to by their position,
  e.g. Fig.~1\,(left). In the caption, the labels (a), (b) \etc should
  precede their description. When referencing specific sub-figures,
  use ``see Fig. 1(a)'' or ``see Figs. 2(b)-(e)''.

\item All figures containing \lhcb data should have \lhcb written on
  them. For preliminary
  results, that should be replaced by ``LHCb preliminary''.
  Figures that only have simulated data should display ``LHCb simulation''.
  Figures that do not depend on LHCb-specific software (\eg only on \pythia)
  should not have any label.


\end{enumerate}


==> fitout.tex <==
\section{Global Minimum Fit Results}
\label{sec:fitout}

\subsection{\DK combination}

\begin{table}
  \caption{Global minimum of the \DK combination}
  \label{tab:dk_fit_out}
  \begin{tabular}{ l | l l l }
    Parameter &  Value & & Uncertainty \\
   \AcpDKK                 &  $-0.002$ & $\pm$ & $0.001$ \\
   \AcpDpipi               &  $0.001$ & $\pm$ & $0.001$ \\
   \Fkkpi0                 &  $0.736$ & $\pm$ & $0.055$ \\
   \Fpipipi0               &  $0.972$ & $\pm$ & $0.017$ \\
   \Fpipipipi              &  $0.746$ & $\pm$ & $0.033$ \\
   \Rdkstz                 &  $1.026$ & $\pm$ & $0.063$ \\
   \dDk3pi                 &  $134.561$ & $\pm$ & $18.284$ (Deg) \\
   \dDkpi                  &  $186.898$ & $\pm$ & $6.711$ (Deg) \\
   \dDkpipi0               &  $198.272$ & $\pm$ & $13.490$ (Deg) \\
   \dDkskpi                &  $342.208$ & $\pm$ & $16.423$ (Deg) \\
   \ddk                    &  $142.632$ & $\pm$ & $5.906$ (Deg) \\
   \ddkpipi                &  $355.980$ & $\pm$ & $17.972$ (Deg) \\
   \ddkstz                 &  $188.626$ & $\pm$ & $20.263$ (Deg) \\
   \ddsk                   &  $348.642$ & $\pm$ & $15.628$ (Deg) \\
   \deltadkstz             &  $0.023$ & $\pm$ & $0.112$ \\
   \g                      &  $72.245$ & $\pm$ & $6.680$ (Deg) \\
   \kDk3pi                 &  $0.377$ & $\pm$ & $0.097$ \\
   \kDkpipi0               &  $0.808$ & $\pm$ & $0.060$ \\
   \kDkskpi                &  $0.950$ & $\pm$ & $0.113$ \\
   \kdkpipi                &  $0.943$ & $\pm$ & $1.047$ \\
   \kdkstz                 &  $0.958$ & $\pm$ & $0.025$ \\
   \ldsk                   &  $0.511$ & $\pm$ & $0.168$ \\
   \phis                   &  $-0.008$ & $\pm$ & $0.039$ \\
   \rDk3pi                 &  $0.055$ & $\pm$ & $0.001$ \\
   \rDkpi                  &  $0.059$ & $\pm$ & $0.000$ \\
   \rDkpipi0               &  $0.045$ & $\pm$ & $0.001$ \\
   \rDkskpi                &  $0.608$ & $\pm$ & $0.010$ \\
   \rdk                    &  $0.102$ & $\pm$ & $0.006$ \\
   \rdkpipi                &  $0.078$ & $\pm$ & $0.034$ \\
   \rdkstz                 &  $0.218$ & $\pm$ & $0.046$ \\
   \xD                     &  $0.004$ & $\pm$ & $0.002$ \\
   \yD                     &  $0.006$ & $\pm$ & $0.001$ \\
  \end{tabular}
\end{table}

\begin{table}
  \caption{Parameter correlation of the \DK combination}
  \label{tab:dk_fit_corr}
  \begin{tabular}{ l | l l l l l l l l l l l l l l l l l l l l l l l l l l l l l l l l }
               & \AcpDKK & \AcpDpipi & \Fkkpi0 & \Fpipipi0 & \Fpipipipi & \Rdkstz & \dDk3pi & \dDkpi & \dDkpipi0 & \dDkskpi &  \ddk & \ddkpipi & \ddkstz & \ddsk & \deltadkstz &    \g & \kDk3pi & \kDkpipi0 & \kDkskpi & \kdkpipi & \kdkstz & \ldsk & \phis & \rDk3pi & \rDkpi & \rDkpipi0 & \rDkskpi &  \rdk & \rdkpipi & \rdkstz &   \xD &   \yD \\
    \AcpDKK    & $\phantom{-}1.000$ & $\phantom{-}0.718$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.003$ & $-0.156$ & $-0.008$ & $-0.003$ & $\phantom{-}0.122$ & $\phantom{-}0.009$ & $\phantom{-}0.006$ & $-0.001$ & $\phantom{-}0.000$ & $-0.008$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.003$ & $-0.032$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.004$ & $-0.003$ & $\phantom{-}0.001$ & $\phantom{-}0.008$ & $-0.032$ & $-0.004$ & $\phantom{-}0.095$ & $-0.128$ \\
    \AcpDpipi  & $\phantom{-}0.718$ & $\phantom{-}1.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.003$ & $-0.132$ & $-0.007$ & $-0.002$ & $\phantom{-}0.102$ & $\phantom{-}0.008$ & $\phantom{-}0.005$ & $-0.001$ & $\phantom{-}0.000$ & $-0.007$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.003$ & $-0.027$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.027$ & $-0.002$ & $\phantom{-}0.001$ & $\phantom{-}0.007$ & $-0.027$ & $-0.003$ & $\phantom{-}0.073$ & $-0.097$ \\
    \Fkkpi0    & $-0.001$ & $-0.001$ & $\phantom{-}1.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.005$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.006$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.001$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.001$ & $\phantom{-}0.004$ \\
    \Fpipipi0  & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.006$ & $-0.001$ & $-0.000$ & $\phantom{-}0.010$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.002$ & $-0.005$ \\
    \Fpipipipi & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}1.000$ & $-0.000$ & $-0.001$ & $-0.005$ & $-0.001$ & $-0.001$ & $\phantom{-}0.012$ & $\phantom{-}0.001$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.008$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.002$ & $-0.001$ & $\phantom{-}0.002$ & $\phantom{-}0.001$ & $-0.004$ \\
    \Rdkstz    & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.001$ & $-0.002$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $-0.010$ & $-0.001$ & $\phantom{-}0.037$ & $-0.003$ & $-0.009$ & $-0.023$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.009$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $-0.012$ & $-0.002$ & $-0.261$ & $\phantom{-}0.001$ & $-0.002$ \\
    \dDk3pi    & $-0.003$ & $-0.003$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}1.000$ & $\phantom{-}0.044$ & $\phantom{-}0.142$ & $\phantom{-}0.001$ & $-0.065$ & $-0.007$ & $\phantom{-}0.003$ & $-0.005$ & $-0.001$ & $-0.032$ & $-0.415$ & $\phantom{-}0.041$ & $-0.001$ & $-0.004$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.104$ & $\phantom{-}0.028$ & $\phantom{-}0.068$ & $\phantom{-}0.001$ & $-0.128$ & $\phantom{-}0.006$ & $-0.006$ & $\phantom{-}0.032$ & $\phantom{-}0.036$ \\
    \dDkpi     & $-0.156$ & $-0.132$ & $\phantom{-}0.005$ & $-0.006$ & $-0.005$ & $-0.002$ & $\phantom{-}0.044$ & $\phantom{-}1.000$ & $\phantom{-}0.047$ & $\phantom{-}0.011$ & $-0.580$ & $-0.142$ & $-0.041$ & $\phantom{-}0.010$ & $\phantom{-}0.000$ & $\phantom{-}0.069$ & $-0.045$ & $\phantom{-}0.006$ & $-0.013$ & $\phantom{-}0.215$ & $-0.000$ & $-0.002$ & $-0.000$ & $\phantom{-}0.012$ & $\phantom{-}0.294$ & $\phantom{-}0.017$ & $\phantom{-}0.008$ & $-0.115$ & $\phantom{-}0.188$ & $\phantom{-}0.026$ & $-0.126$ & $\phantom{-}0.838$ \\
    \dDkpipi0  & $-0.008$ & $-0.007$ & $\phantom{-}0.000$ & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.142$ & $\phantom{-}0.047$ & $\phantom{-}1.000$ & $\phantom{-}0.002$ & $-0.068$ & $-0.007$ & $\phantom{-}0.001$ & $-0.002$ & $-0.001$ & $-0.016$ & $-0.014$ & $\phantom{-}0.227$ & $-0.001$ & $\phantom{-}0.003$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.038$ & $\phantom{-}0.018$ & $\phantom{-}0.338$ & $\phantom{-}0.001$ & $-0.039$ & $\phantom{-}0.008$ & $-0.003$ & $\phantom{-}0.005$ & $\phantom{-}0.039$ \\
    \dDkskpi   & $-0.003$ & $-0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.011$ & $\phantom{-}0.002$ & $\phantom{-}1.000$ & $-0.036$ & $-0.003$ & $\phantom{-}0.005$ & $-0.005$ & $-0.001$ & $-0.038$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.543$ & $-0.012$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.001$ & $\phantom{-}0.002$ & $\phantom{-}0.001$ & $-0.076$ & $-0.016$ & $\phantom{-}0.000$ & $-0.008$ & $-0.003$ & $\phantom{-}0.009$ \\
    \ddk       & $\phantom{-}0.122$ & $\phantom{-}0.102$ & $-0.006$ & $\phantom{-}0.010$ & $\phantom{-}0.012$ & $-0.010$ & $-0.065$ & $-0.580$ & $-0.068$ & $-0.036$ & $\phantom{-}1.000$ & $\phantom{-}0.106$ & $-0.047$ & $\phantom{-}0.062$ & $\phantom{-}0.017$ & $\phantom{-}0.437$ & $\phantom{-}0.017$ & $-0.010$ & $\phantom{-}0.027$ & $\phantom{-}0.045$ & $\phantom{-}0.000$ & $-0.013$ & $-0.003$ & $\phantom{-}0.001$ & $-0.135$ & $-0.023$ & $\phantom{-}0.001$ & $\phantom{-}0.388$ & $-0.088$ & $\phantom{-}0.085$ & $\phantom{-}0.148$ & $-0.492$ \\
    \ddkpipi   & $\phantom{-}0.009$ & $\phantom{-}0.008$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.001$ & $-0.007$ & $-0.142$ & $-0.007$ & $-0.003$ & $\phantom{-}0.106$ & $\phantom{-}1.000$ & $-0.001$ & $\phantom{-}0.005$ & $\phantom{-}0.002$ & $\phantom{-}0.038$ & $\phantom{-}0.002$ & $-0.001$ & $\phantom{-}0.003$ & $\phantom{-}0.043$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $-0.000$ & $-0.033$ & $-0.003$ & $-0.000$ & $\phantom{-}0.043$ & $\phantom{-}0.200$ & $\phantom{-}0.006$ & $\phantom{-}0.035$ & $-0.120$ \\
    \ddkstz    & $\phantom{-}0.006$ & $\phantom{-}0.005$ & $-0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.037$ & $\phantom{-}0.003$ & $-0.041$ & $\phantom{-}0.001$ & $\phantom{-}0.005$ & $-0.047$ & $-0.001$ & $\phantom{-}1.000$ & $-0.021$ & $-0.244$ & $-0.150$ & $\phantom{-}0.011$ & $\phantom{-}0.001$ & $-0.002$ & $-0.062$ & $-0.008$ & $\phantom{-}0.005$ & $\phantom{-}0.001$ & $-0.005$ & $-0.011$ & $\phantom{-}0.000$ & $-0.001$ & $-0.077$ & $-0.015$ & $-0.126$ & $\phantom{-}0.011$ & $-0.034$ \\
    \ddsk      & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $-0.003$ & $-0.005$ & $\phantom{-}0.010$ & $-0.002$ & $-0.005$ & $\phantom{-}0.062$ & $\phantom{-}0.005$ & $-0.021$ & $\phantom{-}1.000$ & $\phantom{-}0.005$ & $\phantom{-}0.142$ & $-0.009$ & $-0.001$ & $\phantom{-}0.003$ & $\phantom{-}0.053$ & $\phantom{-}0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.047$ & $\phantom{-}0.004$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.077$ & $\phantom{-}0.009$ & $\phantom{-}0.030$ & $-0.003$ & $\phantom{-}0.008$ \\
    \deltadkstz & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.009$ & $-0.001$ & $\phantom{-}0.000$ & $-0.001$ & $-0.001$ & $\phantom{-}0.017$ & $\phantom{-}0.002$ & $-0.244$ & $\phantom{-}0.005$ & $\phantom{-}1.000$ & $\phantom{-}0.037$ & $-0.002$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.013$ & $-0.001$ & $-0.001$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.020$ & $\phantom{-}0.002$ & $\phantom{-}0.040$ & $-0.000$ & $\phantom{-}0.000$ \\
    \g         & $-0.008$ & $-0.007$ & $\phantom{-}0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.008$ & $-0.023$ & $-0.032$ & $\phantom{-}0.069$ & $-0.016$ & $-0.038$ & $\phantom{-}0.437$ & $\phantom{-}0.038$ & $-0.150$ & $\phantom{-}0.142$ & $\phantom{-}0.037$ & $\phantom{-}1.000$ & $-0.065$ & $-0.005$ & $\phantom{-}0.018$ & $\phantom{-}0.374$ & $\phantom{-}0.001$ & $-0.030$ & $-0.006$ & $\phantom{-}0.029$ & $\phantom{-}0.021$ & $-0.004$ & $\phantom{-}0.004$ & $\phantom{-}0.541$ & $\phantom{-}0.062$ & $\phantom{-}0.210$ & $-0.022$ & $\phantom{-}0.057$ \\
    \kDk3pi    & $\phantom{-}0.003$ & $\phantom{-}0.003$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.002$ & $-0.415$ & $-0.045$ & $-0.014$ & $\phantom{-}0.002$ & $\phantom{-}0.017$ & $\phantom{-}0.002$ & $\phantom{-}0.011$ & $-0.009$ & $-0.002$ & $-0.065$ & $\phantom{-}1.000$ & $\phantom{-}0.034$ & $-0.000$ & $-0.030$ & $-0.000$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.377$ & $-0.035$ & $-0.017$ & $-0.002$ & $-0.009$ & $-0.010$ & $-0.014$ & $-0.053$ & $-0.037$ \\
    \kDkpipi0  & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.041$ & $\phantom{-}0.006$ & $\phantom{-}0.227$ & $\phantom{-}0.000$ & $-0.010$ & $-0.001$ & $\phantom{-}0.001$ & $-0.001$ & $-0.000$ & $-0.005$ & $\phantom{-}0.034$ & $\phantom{-}1.000$ & $-0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.034$ & $\phantom{-}0.002$ & $-0.048$ & $\phantom{-}0.000$ & $-0.016$ & $\phantom{-}0.001$ & $-0.001$ & $-0.000$ & $\phantom{-}0.005$ \\
    \kDkskpi   & $\phantom{-}0.003$ & $\phantom{-}0.003$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $-0.013$ & $-0.001$ & $-0.543$ & $\phantom{-}0.027$ & $\phantom{-}0.003$ & $-0.002$ & $\phantom{-}0.003$ & $\phantom{-}0.001$ & $\phantom{-}0.018$ & $-0.000$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.004$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $-0.003$ & $-0.000$ & $\phantom{-}0.065$ & $\phantom{-}0.005$ & $-0.002$ & $\phantom{-}0.004$ & $\phantom{-}0.004$ & $-0.011$ \\
    \kdkpipi   & $-0.032$ & $-0.027$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.002$ & $-0.009$ & $-0.004$ & $\phantom{-}0.215$ & $\phantom{-}0.003$ & $-0.012$ & $\phantom{-}0.045$ & $\phantom{-}0.043$ & $-0.062$ & $\phantom{-}0.053$ & $\phantom{-}0.013$ & $\phantom{-}0.374$ & $-0.030$ & $-0.001$ & $\phantom{-}0.004$ & $\phantom{-}1.000$ & $\phantom{-}0.000$ & $-0.011$ & $-0.002$ & $\phantom{-}0.013$ & $\phantom{-}0.055$ & $\phantom{-}0.002$ & $\phantom{-}0.002$ & $\phantom{-}0.173$ & $\phantom{-}0.470$ & $\phantom{-}0.081$ & $-0.056$ & $\phantom{-}0.182$ \\
    \kdkstz    & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.008$ & $\phantom{-}0.000$ & $-0.001$ & $\phantom{-}0.001$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}1.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.006$ & $\phantom{-}0.000$ & $-0.000$ \\
    \ldsk      & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.002$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $-0.013$ & $-0.001$ & $\phantom{-}0.005$ & $\phantom{-}0.003$ & $-0.001$ & $-0.030$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.001$ & $-0.011$ & $-0.000$ & $\phantom{-}1.000$ & $-0.010$ & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $-0.016$ & $-0.002$ & $-0.006$ & $\phantom{-}0.001$ & $-0.002$ \\
    \phis      & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.003$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.047$ & $-0.000$ & $-0.006$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.002$ & $-0.000$ & $-0.010$ & $\phantom{-}1.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.003$ & $-0.000$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ \\
    \rDk3pi    & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.104$ & $\phantom{-}0.012$ & $-0.038$ & $-0.001$ & $\phantom{-}0.001$ & $-0.000$ & $-0.005$ & $\phantom{-}0.004$ & $\phantom{-}0.001$ & $\phantom{-}0.029$ & $-0.377$ & $-0.034$ & $\phantom{-}0.000$ & $\phantom{-}0.013$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.010$ & $-0.044$ & $\phantom{-}0.001$ & $\phantom{-}0.022$ & $\phantom{-}0.003$ & $\phantom{-}0.006$ & $\phantom{-}0.015$ & $\phantom{-}0.010$ \\
    \rDkpi     & $-0.004$ & $-0.027$ & $\phantom{-}0.001$ & $-0.001$ & $-0.001$ & $-0.001$ & $\phantom{-}0.028$ & $\phantom{-}0.294$ & $\phantom{-}0.018$ & $\phantom{-}0.002$ & $-0.135$ & $-0.033$ & $-0.011$ & $\phantom{-}0.003$ & $\phantom{-}0.000$ & $\phantom{-}0.021$ & $-0.035$ & $\phantom{-}0.002$ & $-0.003$ & $\phantom{-}0.055$ & $-0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.010$ & $\phantom{-}1.000$ & $\phantom{-}0.007$ & $\phantom{-}0.011$ & $-0.035$ & $\phantom{-}0.044$ & $\phantom{-}0.006$ & $\phantom{-}0.385$ & $-0.062$ \\
    \rDkpipi0  & $-0.003$ & $-0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.068$ & $\phantom{-}0.017$ & $\phantom{-}0.338$ & $\phantom{-}0.001$ & $-0.023$ & $-0.003$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $-0.004$ & $-0.017$ & $-0.048$ & $-0.000$ & $\phantom{-}0.002$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.044$ & $\phantom{-}0.007$ & $\phantom{-}1.000$ & $\phantom{-}0.000$ & $-0.018$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.003$ & $\phantom{-}0.014$ \\
    \rDkskpi   & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.008$ & $\phantom{-}0.001$ & $-0.076$ & $\phantom{-}0.001$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.004$ & $-0.002$ & $\phantom{-}0.000$ & $\phantom{-}0.065$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.011$ & $\phantom{-}0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.029$ & $\phantom{-}0.009$ \\
    \rdk       & $\phantom{-}0.008$ & $\phantom{-}0.007$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.002$ & $-0.012$ & $-0.128$ & $-0.115$ & $-0.039$ & $-0.016$ & $\phantom{-}0.388$ & $\phantom{-}0.043$ & $-0.077$ & $\phantom{-}0.077$ & $\phantom{-}0.020$ & $\phantom{-}0.541$ & $-0.009$ & $-0.016$ & $\phantom{-}0.005$ & $\phantom{-}0.173$ & $\phantom{-}0.000$ & $-0.016$ & $-0.003$ & $\phantom{-}0.022$ & $-0.035$ & $-0.018$ & $\phantom{-}0.001$ & $\phantom{-}1.000$ & $\phantom{-}0.005$ & $\phantom{-}0.112$ & $\phantom{-}0.023$ & $-0.101$ \\
    \rdkpipi   & $-0.032$ & $-0.027$ & $\phantom{-}0.001$ & $-0.001$ & $-0.001$ & $-0.002$ & $\phantom{-}0.006$ & $\phantom{-}0.188$ & $\phantom{-}0.008$ & $\phantom{-}0.000$ & $-0.088$ & $\phantom{-}0.200$ & $-0.015$ & $\phantom{-}0.009$ & $\phantom{-}0.002$ & $\phantom{-}0.062$ & $-0.010$ & $\phantom{-}0.001$ & $-0.002$ & $\phantom{-}0.470$ & $-0.000$ & $-0.002$ & $-0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.044$ & $\phantom{-}0.003$ & $\phantom{-}0.001$ & $\phantom{-}0.005$ & $\phantom{-}1.000$ & $\phantom{-}0.015$ & $-0.048$ & $\phantom{-}0.159$ \\
    \rdkstz    & $-0.004$ & $-0.003$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.002$ & $-0.261$ & $-0.006$ & $\phantom{-}0.026$ & $-0.003$ & $-0.008$ & $\phantom{-}0.085$ & $\phantom{-}0.006$ & $-0.126$ & $\phantom{-}0.030$ & $\phantom{-}0.040$ & $\phantom{-}0.210$ & $-0.014$ & $-0.001$ & $\phantom{-}0.004$ & $\phantom{-}0.081$ & $-0.006$ & $-0.006$ & $-0.001$ & $\phantom{-}0.006$ & $\phantom{-}0.006$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.112$ & $\phantom{-}0.015$ & $\phantom{-}1.000$ & $-0.008$ & $\phantom{-}0.022$ \\
    \xD        & $\phantom{-}0.095$ & $\phantom{-}0.073$ & $-0.001$ & $\phantom{-}0.002$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.032$ & $-0.126$ & $\phantom{-}0.005$ & $-0.003$ & $\phantom{-}0.148$ & $\phantom{-}0.035$ & $\phantom{-}0.011$ & $-0.003$ & $-0.000$ & $-0.022$ & $-0.053$ & $-0.000$ & $\phantom{-}0.004$ & $-0.056$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.015$ & $\phantom{-}0.385$ & $\phantom{-}0.003$ & $\phantom{-}0.029$ & $\phantom{-}0.023$ & $-0.048$ & $-0.008$ & $\phantom{-}1.000$ & $-0.188$ \\
    \yD        & $-0.128$ & $-0.097$ & $\phantom{-}0.004$ & $-0.005$ & $-0.004$ & $-0.002$ & $\phantom{-}0.036$ & $\phantom{-}0.838$ & $\phantom{-}0.039$ & $\phantom{-}0.009$ & $-0.492$ & $-0.120$ & $-0.034$ & $\phantom{-}0.008$ & $\phantom{-}0.000$ & $\phantom{-}0.057$ & $-0.037$ & $\phantom{-}0.005$ & $-0.011$ & $\phantom{-}0.182$ & $-0.000$ & $-0.002$ & $-0.000$ & $\phantom{-}0.010$ & $-0.062$ & $\phantom{-}0.014$ & $\phantom{-}0.009$ & $-0.101$ & $\phantom{-}0.159$ & $\phantom{-}0.022$ & $-0.188$ & $\phantom{-}1.000$ \\
  \end{tabular}
\end{table}




\subsection{\Dh combination}



==> gammacombo_solution_ckm2016dk_g.tex <==
%SOLUTION 0:

%  combination: ckm2016dk
%  title:       DK CKM 2016
%  date:        Fri Nov 25 20:17:30 2016
%  FCN: 27.5479, EDM: 0.000101221
%  COV quality: 3, status: 0, confirmed: yes

\begin{tabular}{ l | l l l }
  Parameter &  Value & & Uncertainty \\
 \AcpDKK                 &  $-0.002$ & $\pm$ & $0.001$ \\
 \AcpDpipi               &  $0.001$ & $\pm$ & $0.001$ \\
 \Fkkpi0                 &  $0.736$ & $\pm$ & $0.055$ \\
 \Fpipipi0               &  $0.972$ & $\pm$ & $0.017$ \\
 \Fpipipipi              &  $0.746$ & $\pm$ & $0.033$ \\
 \Rdkstz                 &  $1.026$ & $\pm$ & $0.063$ \\
 \dDk3pi                 &  $134.561$ & $\pm$ & $18.284$ (Deg) \\
 \dDkpi                  &  $186.898$ & $\pm$ & $6.711$ (Deg) \\
 \dDkpipi0               &  $198.272$ & $\pm$ & $13.490$ (Deg) \\
 \dDkskpi                &  $342.208$ & $\pm$ & $16.423$ (Deg) \\
 \ddk                    &  $142.632$ & $\pm$ & $5.906$ (Deg) \\
 \ddkpipi                &  $355.980$ & $\pm$ & $17.972$ (Deg) \\
 \ddkstz                 &  $188.626$ & $\pm$ & $20.263$ (Deg) \\
 \ddsk                   &  $348.642$ & $\pm$ & $15.628$ (Deg) \\
 \deltadkstz             &  $0.023$ & $\pm$ & $0.112$ \\
 \g                      &  $72.245$ & $\pm$ & $6.680$ (Deg) \\
 \kDk3pi                 &  $0.377$ & $\pm$ & $0.097$ \\
 \kDkpipi0               &  $0.808$ & $\pm$ & $0.060$ \\
 \kDkskpi                &  $0.950$ & $\pm$ & $0.113$ \\
 \kdkpipi                &  $0.943$ & $\pm$ & $1.047$ \\
 \kdkstz                 &  $0.958$ & $\pm$ & $0.025$ \\
 \ldsk                   &  $0.511$ & $\pm$ & $0.168$ \\
 \phis                   &  $-0.008$ & $\pm$ & $0.039$ \\
 \rDk3pi                 &  $0.055$ & $\pm$ & $0.001$ \\
 \rDkpi                  &  $0.059$ & $\pm$ & $0.000$ \\
 \rDkpipi0               &  $0.045$ & $\pm$ & $0.001$ \\
 \rDkskpi                &  $0.608$ & $\pm$ & $0.010$ \\
 \rdk                    &  $0.102$ & $\pm$ & $0.006$ \\
 \rdkpipi                &  $0.078$ & $\pm$ & $0.034$ \\
 \rdkstz                 &  $0.218$ & $\pm$ & $0.046$ \\
 \xD                     &  $0.004$ & $\pm$ & $0.002$ \\
 \yD                     &  $0.006$ & $\pm$ & $0.001$ \\
\end{tabular}

%Correlation matrix
\begin{tabular}{ l | l l l l l l l l l l l l l l l l l l l l l l l l l l l l l l l l }
             & \AcpDKK & \AcpDpipi & \Fkkpi0 & \Fpipipi0 & \Fpipipipi & \Rdkstz & \dDk3pi & \dDkpi & \dDkpipi0 & \dDkskpi &  \ddk & \ddkpipi & \ddkstz & \ddsk & \deltadkstz &    \g & \kDk3pi & \kDkpipi0 & \kDkskpi & \kdkpipi & \kdkstz & \ldsk & \phis & \rDk3pi & \rDkpi & \rDkpipi0 & \rDkskpi &  \rdk & \rdkpipi & \rdkstz &   \xD &   \yD \\
  \AcpDKK    & $\phantom{-}1.000$ & $\phantom{-}0.718$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.003$ & $-0.156$ & $-0.008$ & $-0.003$ & $\phantom{-}0.122$ & $\phantom{-}0.009$ & $\phantom{-}0.006$ & $-0.001$ & $\phantom{-}0.000$ & $-0.008$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.003$ & $-0.032$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.004$ & $-0.003$ & $\phantom{-}0.001$ & $\phantom{-}0.008$ & $-0.032$ & $-0.004$ & $\phantom{-}0.095$ & $-0.128$ \\
  \AcpDpipi  & $\phantom{-}0.718$ & $\phantom{-}1.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.003$ & $-0.132$ & $-0.007$ & $-0.002$ & $\phantom{-}0.102$ & $\phantom{-}0.008$ & $\phantom{-}0.005$ & $-0.001$ & $\phantom{-}0.000$ & $-0.007$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.003$ & $-0.027$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.027$ & $-0.002$ & $\phantom{-}0.001$ & $\phantom{-}0.007$ & $-0.027$ & $-0.003$ & $\phantom{-}0.073$ & $-0.097$ \\
  \Fkkpi0    & $-0.001$ & $-0.001$ & $\phantom{-}1.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.005$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.006$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.001$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.001$ & $\phantom{-}0.004$ \\
  \Fpipipi0  & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.006$ & $-0.001$ & $-0.000$ & $\phantom{-}0.010$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.002$ & $-0.005$ \\
  \Fpipipipi & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}1.000$ & $-0.000$ & $-0.001$ & $-0.005$ & $-0.001$ & $-0.001$ & $\phantom{-}0.012$ & $\phantom{-}0.001$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.008$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.002$ & $-0.001$ & $\phantom{-}0.002$ & $\phantom{-}0.001$ & $-0.004$ \\
  \Rdkstz    & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.001$ & $-0.002$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $-0.010$ & $-0.001$ & $\phantom{-}0.037$ & $-0.003$ & $-0.009$ & $-0.023$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.009$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $-0.012$ & $-0.002$ & $-0.261$ & $\phantom{-}0.001$ & $-0.002$ \\
  \dDk3pi    & $-0.003$ & $-0.003$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}1.000$ & $\phantom{-}0.044$ & $\phantom{-}0.142$ & $\phantom{-}0.001$ & $-0.065$ & $-0.007$ & $\phantom{-}0.003$ & $-0.005$ & $-0.001$ & $-0.032$ & $-0.415$ & $\phantom{-}0.041$ & $-0.001$ & $-0.004$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.104$ & $\phantom{-}0.028$ & $\phantom{-}0.068$ & $\phantom{-}0.001$ & $-0.128$ & $\phantom{-}0.006$ & $-0.006$ & $\phantom{-}0.032$ & $\phantom{-}0.036$ \\
  \dDkpi     & $-0.156$ & $-0.132$ & $\phantom{-}0.005$ & $-0.006$ & $-0.005$ & $-0.002$ & $\phantom{-}0.044$ & $\phantom{-}1.000$ & $\phantom{-}0.047$ & $\phantom{-}0.011$ & $-0.580$ & $-0.142$ & $-0.041$ & $\phantom{-}0.010$ & $\phantom{-}0.000$ & $\phantom{-}0.069$ & $-0.045$ & $\phantom{-}0.006$ & $-0.013$ & $\phantom{-}0.215$ & $-0.000$ & $-0.002$ & $-0.000$ & $\phantom{-}0.012$ & $\phantom{-}0.294$ & $\phantom{-}0.017$ & $\phantom{-}0.008$ & $-0.115$ & $\phantom{-}0.188$ & $\phantom{-}0.026$ & $-0.126$ & $\phantom{-}0.838$ \\
  \dDkpipi0  & $-0.008$ & $-0.007$ & $\phantom{-}0.000$ & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.142$ & $\phantom{-}0.047$ & $\phantom{-}1.000$ & $\phantom{-}0.002$ & $-0.068$ & $-0.007$ & $\phantom{-}0.001$ & $-0.002$ & $-0.001$ & $-0.016$ & $-0.014$ & $\phantom{-}0.227$ & $-0.001$ & $\phantom{-}0.003$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.038$ & $\phantom{-}0.018$ & $\phantom{-}0.338$ & $\phantom{-}0.001$ & $-0.039$ & $\phantom{-}0.008$ & $-0.003$ & $\phantom{-}0.005$ & $\phantom{-}0.039$ \\
  \dDkskpi   & $-0.003$ & $-0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.011$ & $\phantom{-}0.002$ & $\phantom{-}1.000$ & $-0.036$ & $-0.003$ & $\phantom{-}0.005$ & $-0.005$ & $-0.001$ & $-0.038$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.543$ & $-0.012$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.001$ & $\phantom{-}0.002$ & $\phantom{-}0.001$ & $-0.076$ & $-0.016$ & $\phantom{-}0.000$ & $-0.008$ & $-0.003$ & $\phantom{-}0.009$ \\
  \ddk       & $\phantom{-}0.122$ & $\phantom{-}0.102$ & $-0.006$ & $\phantom{-}0.010$ & $\phantom{-}0.012$ & $-0.010$ & $-0.065$ & $-0.580$ & $-0.068$ & $-0.036$ & $\phantom{-}1.000$ & $\phantom{-}0.106$ & $-0.047$ & $\phantom{-}0.062$ & $\phantom{-}0.017$ & $\phantom{-}0.437$ & $\phantom{-}0.017$ & $-0.010$ & $\phantom{-}0.027$ & $\phantom{-}0.045$ & $\phantom{-}0.000$ & $-0.013$ & $-0.003$ & $\phantom{-}0.001$ & $-0.135$ & $-0.023$ & $\phantom{-}0.001$ & $\phantom{-}0.388$ & $-0.088$ & $\phantom{-}0.085$ & $\phantom{-}0.148$ & $-0.492$ \\
  \ddkpipi   & $\phantom{-}0.009$ & $\phantom{-}0.008$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.001$ & $-0.007$ & $-0.142$ & $-0.007$ & $-0.003$ & $\phantom{-}0.106$ & $\phantom{-}1.000$ & $-0.001$ & $\phantom{-}0.005$ & $\phantom{-}0.002$ & $\phantom{-}0.038$ & $\phantom{-}0.002$ & $-0.001$ & $\phantom{-}0.003$ & $\phantom{-}0.043$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $-0.000$ & $-0.033$ & $-0.003$ & $-0.000$ & $\phantom{-}0.043$ & $\phantom{-}0.200$ & $\phantom{-}0.006$ & $\phantom{-}0.035$ & $-0.120$ \\
  \ddkstz    & $\phantom{-}0.006$ & $\phantom{-}0.005$ & $-0.000$ & $-0.000$ & $-0.001$ & $\phantom{-}0.037$ & $\phantom{-}0.003$ & $-0.041$ & $\phantom{-}0.001$ & $\phantom{-}0.005$ & $-0.047$ & $-0.001$ & $\phantom{-}1.000$ & $-0.021$ & $-0.244$ & $-0.150$ & $\phantom{-}0.011$ & $\phantom{-}0.001$ & $-0.002$ & $-0.062$ & $-0.008$ & $\phantom{-}0.005$ & $\phantom{-}0.001$ & $-0.005$ & $-0.011$ & $\phantom{-}0.000$ & $-0.001$ & $-0.077$ & $-0.015$ & $-0.126$ & $\phantom{-}0.011$ & $-0.034$ \\
  \ddsk      & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $-0.003$ & $-0.005$ & $\phantom{-}0.010$ & $-0.002$ & $-0.005$ & $\phantom{-}0.062$ & $\phantom{-}0.005$ & $-0.021$ & $\phantom{-}1.000$ & $\phantom{-}0.005$ & $\phantom{-}0.142$ & $-0.009$ & $-0.001$ & $\phantom{-}0.003$ & $\phantom{-}0.053$ & $\phantom{-}0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.047$ & $\phantom{-}0.004$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.077$ & $\phantom{-}0.009$ & $\phantom{-}0.030$ & $-0.003$ & $\phantom{-}0.008$ \\
  \deltadkstz & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.009$ & $-0.001$ & $\phantom{-}0.000$ & $-0.001$ & $-0.001$ & $\phantom{-}0.017$ & $\phantom{-}0.002$ & $-0.244$ & $\phantom{-}0.005$ & $\phantom{-}1.000$ & $\phantom{-}0.037$ & $-0.002$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.013$ & $-0.001$ & $-0.001$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.020$ & $\phantom{-}0.002$ & $\phantom{-}0.040$ & $-0.000$ & $\phantom{-}0.000$ \\
  \g         & $-0.008$ & $-0.007$ & $\phantom{-}0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.008$ & $-0.023$ & $-0.032$ & $\phantom{-}0.069$ & $-0.016$ & $-0.038$ & $\phantom{-}0.437$ & $\phantom{-}0.038$ & $-0.150$ & $\phantom{-}0.142$ & $\phantom{-}0.037$ & $\phantom{-}1.000$ & $-0.065$ & $-0.005$ & $\phantom{-}0.018$ & $\phantom{-}0.374$ & $\phantom{-}0.001$ & $-0.030$ & $-0.006$ & $\phantom{-}0.029$ & $\phantom{-}0.021$ & $-0.004$ & $\phantom{-}0.004$ & $\phantom{-}0.541$ & $\phantom{-}0.062$ & $\phantom{-}0.210$ & $-0.022$ & $\phantom{-}0.057$ \\
  \kDk3pi    & $\phantom{-}0.003$ & $\phantom{-}0.003$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.002$ & $-0.415$ & $-0.045$ & $-0.014$ & $\phantom{-}0.002$ & $\phantom{-}0.017$ & $\phantom{-}0.002$ & $\phantom{-}0.011$ & $-0.009$ & $-0.002$ & $-0.065$ & $\phantom{-}1.000$ & $\phantom{-}0.034$ & $-0.000$ & $-0.030$ & $-0.000$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.377$ & $-0.035$ & $-0.017$ & $-0.002$ & $-0.009$ & $-0.010$ & $-0.014$ & $-0.053$ & $-0.037$ \\
  \kDkpipi0  & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.041$ & $\phantom{-}0.006$ & $\phantom{-}0.227$ & $\phantom{-}0.000$ & $-0.010$ & $-0.001$ & $\phantom{-}0.001$ & $-0.001$ & $-0.000$ & $-0.005$ & $\phantom{-}0.034$ & $\phantom{-}1.000$ & $-0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.034$ & $\phantom{-}0.002$ & $-0.048$ & $\phantom{-}0.000$ & $-0.016$ & $\phantom{-}0.001$ & $-0.001$ & $-0.000$ & $\phantom{-}0.005$ \\
  \kDkskpi   & $\phantom{-}0.003$ & $\phantom{-}0.003$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.001$ & $-0.013$ & $-0.001$ & $-0.543$ & $\phantom{-}0.027$ & $\phantom{-}0.003$ & $-0.002$ & $\phantom{-}0.003$ & $\phantom{-}0.001$ & $\phantom{-}0.018$ & $-0.000$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.004$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.000$ & $-0.003$ & $-0.000$ & $\phantom{-}0.065$ & $\phantom{-}0.005$ & $-0.002$ & $\phantom{-}0.004$ & $\phantom{-}0.004$ & $-0.011$ \\
  \kdkpipi   & $-0.032$ & $-0.027$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.002$ & $-0.009$ & $-0.004$ & $\phantom{-}0.215$ & $\phantom{-}0.003$ & $-0.012$ & $\phantom{-}0.045$ & $\phantom{-}0.043$ & $-0.062$ & $\phantom{-}0.053$ & $\phantom{-}0.013$ & $\phantom{-}0.374$ & $-0.030$ & $-0.001$ & $\phantom{-}0.004$ & $\phantom{-}1.000$ & $\phantom{-}0.000$ & $-0.011$ & $-0.002$ & $\phantom{-}0.013$ & $\phantom{-}0.055$ & $\phantom{-}0.002$ & $\phantom{-}0.002$ & $\phantom{-}0.173$ & $\phantom{-}0.470$ & $\phantom{-}0.081$ & $-0.056$ & $\phantom{-}0.182$ \\
  \kdkstz    & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.008$ & $\phantom{-}0.000$ & $-0.001$ & $\phantom{-}0.001$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}1.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.006$ & $\phantom{-}0.000$ & $-0.000$ \\
  \ldsk      & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $-0.002$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $-0.013$ & $-0.001$ & $\phantom{-}0.005$ & $\phantom{-}0.003$ & $-0.001$ & $-0.030$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.001$ & $-0.011$ & $-0.000$ & $\phantom{-}1.000$ & $-0.010$ & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $-0.016$ & $-0.002$ & $-0.006$ & $\phantom{-}0.001$ & $-0.002$ \\
  \phis      & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.003$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.047$ & $-0.000$ & $-0.006$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.002$ & $-0.000$ & $-0.010$ & $\phantom{-}1.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.000$ & $-0.003$ & $-0.000$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ \\
  \rDk3pi    & $-0.001$ & $-0.001$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.000$ & $-0.001$ & $-0.104$ & $\phantom{-}0.012$ & $-0.038$ & $-0.001$ & $\phantom{-}0.001$ & $-0.000$ & $-0.005$ & $\phantom{-}0.004$ & $\phantom{-}0.001$ & $\phantom{-}0.029$ & $-0.377$ & $-0.034$ & $\phantom{-}0.000$ & $\phantom{-}0.013$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.010$ & $-0.044$ & $\phantom{-}0.001$ & $\phantom{-}0.022$ & $\phantom{-}0.003$ & $\phantom{-}0.006$ & $\phantom{-}0.015$ & $\phantom{-}0.010$ \\
  \rDkpi     & $-0.004$ & $-0.027$ & $\phantom{-}0.001$ & $-0.001$ & $-0.001$ & $-0.001$ & $\phantom{-}0.028$ & $\phantom{-}0.294$ & $\phantom{-}0.018$ & $\phantom{-}0.002$ & $-0.135$ & $-0.033$ & $-0.011$ & $\phantom{-}0.003$ & $\phantom{-}0.000$ & $\phantom{-}0.021$ & $-0.035$ & $\phantom{-}0.002$ & $-0.003$ & $\phantom{-}0.055$ & $-0.000$ & $-0.001$ & $-0.000$ & $\phantom{-}0.010$ & $\phantom{-}1.000$ & $\phantom{-}0.007$ & $\phantom{-}0.011$ & $-0.035$ & $\phantom{-}0.044$ & $\phantom{-}0.006$ & $\phantom{-}0.385$ & $-0.062$ \\
  \rDkpipi0  & $-0.003$ & $-0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.068$ & $\phantom{-}0.017$ & $\phantom{-}0.338$ & $\phantom{-}0.001$ & $-0.023$ & $-0.003$ & $\phantom{-}0.000$ & $-0.001$ & $-0.000$ & $-0.004$ & $-0.017$ & $-0.048$ & $-0.000$ & $\phantom{-}0.002$ & $-0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.044$ & $\phantom{-}0.007$ & $\phantom{-}1.000$ & $\phantom{-}0.000$ & $-0.018$ & $\phantom{-}0.003$ & $-0.001$ & $\phantom{-}0.003$ & $\phantom{-}0.014$ \\
  \rDkskpi   & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $\phantom{-}0.000$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.008$ & $\phantom{-}0.001$ & $-0.076$ & $\phantom{-}0.001$ & $-0.000$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.004$ & $-0.002$ & $\phantom{-}0.000$ & $\phantom{-}0.065$ & $\phantom{-}0.002$ & $\phantom{-}0.000$ & $-0.000$ & $-0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.011$ & $\phantom{-}0.000$ & $\phantom{-}1.000$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.029$ & $\phantom{-}0.009$ \\
  \rdk       & $\phantom{-}0.008$ & $\phantom{-}0.007$ & $\phantom{-}0.001$ & $-0.000$ & $\phantom{-}0.002$ & $-0.012$ & $-0.128$ & $-0.115$ & $-0.039$ & $-0.016$ & $\phantom{-}0.388$ & $\phantom{-}0.043$ & $-0.077$ & $\phantom{-}0.077$ & $\phantom{-}0.020$ & $\phantom{-}0.541$ & $-0.009$ & $-0.016$ & $\phantom{-}0.005$ & $\phantom{-}0.173$ & $\phantom{-}0.000$ & $-0.016$ & $-0.003$ & $\phantom{-}0.022$ & $-0.035$ & $-0.018$ & $\phantom{-}0.001$ & $\phantom{-}1.000$ & $\phantom{-}0.005$ & $\phantom{-}0.112$ & $\phantom{-}0.023$ & $-0.101$ \\
  \rdkpipi   & $-0.032$ & $-0.027$ & $\phantom{-}0.001$ & $-0.001$ & $-0.001$ & $-0.002$ & $\phantom{-}0.006$ & $\phantom{-}0.188$ & $\phantom{-}0.008$ & $\phantom{-}0.000$ & $-0.088$ & $\phantom{-}0.200$ & $-0.015$ & $\phantom{-}0.009$ & $\phantom{-}0.002$ & $\phantom{-}0.062$ & $-0.010$ & $\phantom{-}0.001$ & $-0.002$ & $\phantom{-}0.470$ & $-0.000$ & $-0.002$ & $-0.000$ & $\phantom{-}0.003$ & $\phantom{-}0.044$ & $\phantom{-}0.003$ & $\phantom{-}0.001$ & $\phantom{-}0.005$ & $\phantom{-}1.000$ & $\phantom{-}0.015$ & $-0.048$ & $\phantom{-}0.159$ \\
  \rdkstz    & $-0.004$ & $-0.003$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.002$ & $-0.261$ & $-0.006$ & $\phantom{-}0.026$ & $-0.003$ & $-0.008$ & $\phantom{-}0.085$ & $\phantom{-}0.006$ & $-0.126$ & $\phantom{-}0.030$ & $\phantom{-}0.040$ & $\phantom{-}0.210$ & $-0.014$ & $-0.001$ & $\phantom{-}0.004$ & $\phantom{-}0.081$ & $-0.006$ & $-0.006$ & $-0.001$ & $\phantom{-}0.006$ & $\phantom{-}0.006$ & $-0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.112$ & $\phantom{-}0.015$ & $\phantom{-}1.000$ & $-0.008$ & $\phantom{-}0.022$ \\
  \xD        & $\phantom{-}0.095$ & $\phantom{-}0.073$ & $-0.001$ & $\phantom{-}0.002$ & $\phantom{-}0.001$ & $\phantom{-}0.001$ & $\phantom{-}0.032$ & $-0.126$ & $\phantom{-}0.005$ & $-0.003$ & $\phantom{-}0.148$ & $\phantom{-}0.035$ & $\phantom{-}0.011$ & $-0.003$ & $-0.000$ & $-0.022$ & $-0.053$ & $-0.000$ & $\phantom{-}0.004$ & $-0.056$ & $\phantom{-}0.000$ & $\phantom{-}0.001$ & $\phantom{-}0.000$ & $\phantom{-}0.015$ & $\phantom{-}0.385$ & $\phantom{-}0.003$ & $\phantom{-}0.029$ & $\phantom{-}0.023$ & $-0.048$ & $-0.008$ & $\phantom{-}1.000$ & $-0.188$ \\
  \yD        & $-0.128$ & $-0.097$ & $\phantom{-}0.004$ & $-0.005$ & $-0.004$ & $-0.002$ & $\phantom{-}0.036$ & $\phantom{-}0.838$ & $\phantom{-}0.039$ & $\phantom{-}0.009$ & $-0.492$ & $-0.120$ & $-0.034$ & $\phantom{-}0.008$ & $\phantom{-}0.000$ & $\phantom{-}0.057$ & $-0.037$ & $\phantom{-}0.005$ & $-0.011$ & $\phantom{-}0.182$ & $-0.000$ & $-0.002$ & $-0.000$ & $\phantom{-}0.010$ & $-0.062$ & $\phantom{-}0.014$ & $\phantom{-}0.009$ & $-0.101$ & $\phantom{-}0.159$ & $\phantom{-}0.022$ & $-0.188$ & $\phantom{-}1.000$ \\
\end{tabular}



==> ggsz-dkstz_syst.tex <==
\begin{tabular}{ l |cccc}
\hline
                & \xmdkst & \ymdkst & \xpdkst & \ypdkst\\
\hline
\xmdkst         &       1 &       0 &       0 &       0  \\
\ymdkst         &       0 &       1 &       0 &       0  \\
\xpdkst         &       0 &       0 &       1 &       0  \\
\ypdkst         &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> gls_stat.tex <==
\begin{tabular}{ l |ccc}
\hline
                & \RfavsupDkKskpi & \AfavDkKskpi & \AsupDkKskpi\\
\hline
\RfavsupDkKskpi &       1 &       0 &       0  \\
\AfavDkKskpi    &       0 &       1 &       0  \\
\AsupDkKskpi    &       0 &       0 &       1  \\
\hline
\end{tabular}


==> gls_syst.tex <==
\begin{tabular}{ l |ccc}
\hline
                & \RfavsupDkKskpi & \AfavDkKskpi & \AsupDkKskpi\\
\hline
\RfavsupDkKskpi &       1 &       0 &       0  \\
\AfavDkKskpi    &       0 &       1 &       0  \\
\AsupDkKskpi    &       0 &       0 &       1  \\
\hline
\end{tabular}


==> glwads-dhpipi-hh_stat.tex <==
\begin{tabular}{ l |ccccccccccc}
\hline
                & \RcpDkpipi & \AfavDkpipiKpi & \AfavDpipipiKpi & \AcpDkpipiKK & \AcpDkpipiPipi & \AcpDpipipiKK & \AcpDpipipiPipi & \RpDkpipiKpi & \RmDkpipiKpi & \RpDpipipiKpi & \RmDpipipiKpi\\
\hline
\RcpDkpipi      &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AfavDkpipiKpi  &       0 &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AfavDpipipiKpi &       0 &       0 &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AcpDkpipiKK    &       0 &       0 &       0 &       1 &   0.200 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AcpDkpipiPipi  &       0 &       0 &       0 &   0.200 &       1 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AcpDpipipiKK   &       0 &       0 &       0 &       0 &       0 &       1 &   0.080 &       0 &       0 &       0 &       0  \\
\AcpDpipipiPipi &       0 &       0 &       0 &       0 &       0 &   0.080 &       1 &       0 &       0 &       0 &       0  \\
\RpDkpipiKpi    &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0 &       0 &       0  \\
\RmDkpipiKpi    &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0 &       0  \\
\RpDpipipiKpi   &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0  \\
\RmDpipipiKpi   &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> glwads-dhpipi-hh_syst.tex <==
\begin{tabular}{ l |ccccccccccc}
\hline
                & \RcpDkpipi & \AfavDkpipiKpi & \AfavDpipipiKpi & \AcpDkpipiKK & \AcpDkpipiPipi & \AcpDpipipiKK & \AcpDpipipiPipi & \RpDkpipiKpi & \RmDkpipiKpi & \RpDpipipiKpi & \RmDpipipiKpi\\
\hline
\RcpDkpipi      &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AfavDkpipiKpi  &       0 &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AfavDpipipiKpi &       0 &       0 &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AcpDkpipiKK    &       0 &       0 &       0 &       1 &       0 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AcpDkpipiPipi  &       0 &       0 &       0 &       0 &       1 &       0 &       0 &       0 &       0 &       0 &       0  \\
\AcpDpipipiKK   &       0 &       0 &       0 &       0 &       0 &       1 &       0 &       0 &       0 &       0 &       0  \\
\AcpDpipipiPipi &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0 &       0 &       0 &       0  \\
\RpDkpipiKpi    &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0 &       0 &       0  \\
\RmDkpipiKpi    &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0 &       0  \\
\RpDpipipiKpi   &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1 &       0  \\
\RmDpipipiKpi   &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> glwads-dk-hh.tex <==
\begin{alignat}{3}
& \AadsDK        & \;=&\;            -0.403\phantom{0}  \;\pm\; & \phantom{0}0.056 \;\pm\; & 0.011\,, \nonumber \\
& \AcpDkKK         & \;=&\;  \phantom{-0}0.087\phantom{0}  \;\pm\; & \phantom{0}0.020 \;\pm\; & 0.008\,, \nonumber \\
& \AcpDkPipi       & \;=&\;  \phantom{-0}0.128\phantom{0}  \;\pm\; & \phantom{0}0.037 \;\pm\; & 0.012\,, \nonumber \\
& \AfavDkKpi       & \;=&\;            -0.0194            \;\pm\; & 0.0072 \;\pm\; & 0.0060\,, \nonumber \\
& \RadsDK          & \;=&\;  \phantom{-0}0.0188            \;\pm\; & 0.0011 \;\pm\; & 0.0010\,, \nonumber \\
& \RCPKK           & \;=&\;  \phantom{-0}0.968\phantom{0}  \;\pm\; & \phantom{0}0.022 \;\pm\; & 0.021 \;\pm\; 0.010 \,, \nonumber \\
& \RCPPiPi         & \;=&\;  \phantom{-0}1.002\phantom{0}  \;\pm\; & \phantom{0}0.040 \;\pm\; & 0.026 \;\pm\; 0.010 \,, \nonumber
\end{alignat}


==> glwads-dk-hh_stat.tex <==
\begin{tabular}{ l |ccccccc}
\hline
                & \AadsDK & \AcpDkKK & \AcpDkPipi & \AfavDkKpi & \RadsDK & \RCPKK & \RCPPiPi\\
\hline
\AadsDK         &   $    1$ &  $ 0.002$ &  $ 0.001$ &   $0.008$ &  $ 0.102$ &  $     0$ &  $     0$  \\
\AcpDkKK        &   $0.002$ &  $     1$ &  $ 0.004$ &   $0.024$ &  $     0$ &  $-0.014$ &  $     0$  \\
\AcpDkPipi      &   $0.001$ &  $ 0.004$ &  $     1$ &   $0.014$ &  $-0.001$ &  $     0$ &  $-0.038$  \\
\AfavDkKpi      &   $0.008$ &  $ 0.024$ &  $ 0.014$ &   $    1$ &  $     0$ &  $     0$ &  $     0$  \\
\RadsDK         &   $0.102$ &  $     0$ &  $-0.001$ &   $    0$ &  $     1$ &  $ 0.040$ &  $ 0.025$  \\
\RCPKK          &   $    0$ &  $-$0.014 &  $     0$ &   $    0$ &  $ 0.040$ &  $     1$ &  $ 0.060$  \\
\RCPPiPi        &   $    0$ &  $     0$ &  $-0.038$ &   $    0$ &  $ 0.025$ &  $ 0.060$ &  $     1$  \\
\hline
\end{tabular}


==> glwads-dk-hh_syst.tex <==
\begin{tabular}{ l |ccccccc}
\hline
                & \AadsDK & \AcpDkKK & \AcpDkPipi & \AfavDkKpi & \RadsDK & \RCPKK & \RCPPiPi\\
\hline
\AadsDK         &  $    1$ &  $-0.06$ &  $ 0.27$ &  $ 0.09$ &  $ 0.78$ &  $ 0.23$ &  $-0.04$  \\
\AcpDkKK        &  $-0.06$ &  $    1$ &  $-0.02$ &  $ 0.09$ &  $-0.10$ &  $-0.28$ &  $ 0.03$  \\
\AcpDkPipi      &  $ 0.27$ &  $-0.02$ &  $    1$ &  $-0.01$ &  $ 0.35$ &  $ 0.11$ &  $-0.22$  \\
\AfavDkKpi      &  $ 0.09$ &  $ 0.09$ &  $-0.01$ &  $    1$ &  $-0.11$ &  $-0.02$ &  $-0.01$  \\
\RadsDK         &  $ 0.78$ &  $-0.10$ &  $ 0.35$ &  $-0.11$ &  $    1$ &  $ 0.33$ &  $-0.14$  \\
\RCPKK          &  $ 0.23$ &  $-0.28$ &  $ 0.11$ &  $-0.02$ &  $ 0.33$ &  $    1$ &  $ 0.17$  \\
\RCPPiPi        &  $-0.04$ &  $ 0.03$ &  $-0.22$ &  $-0.01$ &  $-0.14$ &  $ 0.17$ &  $    1$  \\
\hline
\end{tabular}


==> glwads-dk-hhpiz.tex <==
\begin{alignat}{3}
& \AadsDKkpp            & \;=&\;  \phantom{0}-0.20  \;\pm\; & \phantom{00}0.27 \;\pm\; & 0.04\,, \nonumber \\
& \AcpDkKKPiz           & \;=&\;  \phantom{-00}0.30  \;\pm\; & \phantom{00}0.20 \;\pm\; & 0.02\,, \nonumber \\
& \AcpDkPiPiPiz         & \;=&\;  \phantom{-0}0.054  \;\pm\; & \phantom{0}0.091 \;\pm\; & 0.011\,, \nonumber \\
& \AfavDkKPiPiz         & \;=&\;  \phantom{-0}0.010  \;\pm\; & \phantom{0}0.026 \;\pm\; & 0.005\,, \nonumber \\
& \RadsDKkpp            & \;=&\;  \phantom{-}0.0140  \;\pm\; & 0.0047 \;\pm\; & 0.0021\,, \nonumber \\
& \RCPKKPiz             & \;=&\;  \phantom{-00}0.95  \;\pm\; & \phantom{00}0.22 \;\pm\; & 0.05\,, \nonumber \\
& \RCPPiPiPiz           & \;=&\;  \phantom{-00}0.98  \;\pm\; & \phantom{00}0.11 \;\pm\; & 0.05\,, \nonumber
\end{alignat}


==> glwads-dk-hhpiz_stat.tex <==
\begin{tabular}{ l |ccccccc}
\hline
                & \AadsDKkpp & \AcpDkKKPiz & \AcpDkPiPiPiz & \AfavDkKPiPiz & \RadsDKkpp & \RCPKKPiz & \RCPPiPiPiz\\
\hline
\AadsDKkpp      &       1 &  $     0$ &  $     0$ &   0.010 &   0.130 &  $     0$ &  $     0$  \\
\AcpDkKKPiz     &       0 &  $     1$ &  $     0$ &   0.010 &       0 &  $-0.200$ &  $-0.010$  \\
\AcpDkPiPiPiz   &       0 &  $     0$ &  $     1$ &   0.020 &       0 &  $     0$ &  $-0.040$  \\
\AfavDkKPiPiz   &   0.010 &  $ 0.010$ &  $ 0.020$ &       1 &       0 &  $     0$ &  $     0$  \\
\RadsDKkpp      &   0.130 &  $     0$ &  $     0$ &       0 &       1 &  $     0$ &  $ 0.010$  \\
\RCPKKPiz       &       0 &  $-0.200$ &  $     0$ &       0 &       0 &  $     1$ &  $ 0.020$  \\
\RCPPiPiPiz     &       0 &  $-0.010$ &  $-0.040$ &       0 &   0.010 &  $ 0.020$ &  $     1$  \\
\hline
\end{tabular}


==> glwads-dk-hhpiz_syst.tex <==
\begin{tabular}{ l |ccccccc}
\hline
                & \AadsDKkpp & \AcpDkKKPiz & \AcpDkPiPiPiz & \AfavDkKPiPiz & \RadsDKkpp & \RCPKKPiz & \RCPPiPiPiz\\
\hline
\AadsDKkpp      &  $     1$ &  $ 0.070$ &  $ 0.070$ &  $-0.160$ &  $ 0.810$ &  $ 0.020$ &  $ 0.130$  \\
\AcpDkKKPiz     &  $ 0.070$ &  $     1$ &  $ 0.770$ &  $ 0.050$ &  $ 0.080$ &  $-0.330$ &  $-0.180$  \\
\AcpDkPiPiPiz   &  $ 0.070$ &  $ 0.770$ &  $     1$ &  $-0.060$ &  $ 0.130$ &  $-0.140$ &  $-0.250$  \\
\AfavDkKPiPiz   &  $-0.160$ &  $ 0.050$ &  $-0.060$ &  $     1$ &  $-0.050$ &  $ 0.040$ &  $     0$  \\
\RadsDKkpp      &  $ 0.810$ &  $ 0.080$ &  $ 0.130$ &  $-0.050$ &  $     1$ &  $-0.030$ &  $-0.020$  \\
\RCPKKPiz       &  $ 0.020$ &  $-0.330$ &  $-0.140$ &  $ 0.040$ &  $-0.030$ &  $     1$ &  $ 0.380$  \\
\RCPPiPiPiz     &  $ 0.130$ &  $-0.180$ &  $-0.250$ &  $     0$ &  $-0.020$ &  $ 0.380$ &  $     1$  \\
\hline
\end{tabular}


==> glwads-dk-hpipipi.tex <==
\begin{alignat}{3}
& \AadsDKKppp           & \;=&\;  -0.313 \;\pm\; & \phantom{0}0.102 \;\pm\; & 0.038\,, \nonumber \\
& \AcpDKpppp            & \;=&\;  \phantom{-0}0.100  \;\pm\; & \phantom{0}0.034 \;\pm\; & 0.018\,, \nonumber \\
& \AfavDkKppp           & \;=&\;  \phantom{-0}0.000  \;\pm\; & \phantom{0}0.012 \;\pm\; & 0.002\,, \nonumber \\
& \RadsDKKppp           & \;=&\;  \phantom{-}0.0140  \;\pm\; & 0.0015 \;\pm\; & 0.0006\,, \nonumber \\
& \RCPpppp              & \;=&\;  \phantom{-0}0.975  \;\pm\; & \phantom{0}0.037 \;\pm\; & 0.019 \;\pm\; 0.005 \,, \nonumber
\end{alignat}


==> glwads-dk-hpipipi_stat.tex <==
\begin{tabular}{ l |ccccc}
\hline
                & \AadsDKKppp & \AcpDKpppp & \AfavDkKppp & \RadsDKKppp & \RCPpppp\\
\hline
\AadsDKKppp     &  $     1$ &  $ 0.002$ &   $0.006$ &  $ 0.082$ &  $ 0.002$  \\
\AcpDKpppp      &  $ 0.002$ &  $     1$ &   $0.024$ &  $-0.001$ &  $-0.018$  \\
\AfavDkKppp     &  $ 0.006$ &  $ 0.024$ &   $    1$ &  $     0$ &  $     0$  \\
\RadsDKKppp     &  $ 0.082$ &  $-0.001$ &   $    0$ &  $     1$ &  $ 0.041$  \\
\RCPpppp        &  $ 0.002$ &  $-0.018$ &   $    0$ &  $ 0.041$ &  $     1$  \\
\hline
\end{tabular}


==> glwads-dk-hpipipi_syst.tex <==
\begin{tabular}{ l |ccccc}
\hline
                & \AadsDKKppp & \AcpDKpppp & \AfavDkKppp & \RadsDKKppp & \RCPpppp\\
\hline
\AadsDKKppp     &  $     1$ &  $-0.040$ &   $0.020$ &   $0.870$ &  $-0.040$  \\
\AcpDKpppp      &  $-0.040$ &  $     1$ &   $0.090$ &   $0.030$ &  $ 0.070$  \\
\AfavDkKppp     &  $ 0.020$ &  $ 0.090$ &   $    1$ &   $0.020$ &  $ 0.020$  \\
\RadsDKKppp     &  $ 0.870$ &  $ 0.030$ &   $0.020$ &   $    1$ &  $ 0.040$  \\
\RCPpppp        &  $-0.040$ &  $ 0.070$ &   $0.020$ &   $0.040$ &  $     1$  \\
\hline
\end{tabular}


==> glwads-dkpipi-hh.tex <==
\begin{alignat}{3}
& \RcpDkpipi            & \;=\;  \phantom{-0}1.040  \;\pm\; & \phantom{0}0.064\,, \nonumber \\
& \AfavDkpipiKpi        & \;=\;  \phantom{-0}0.013  \;\pm\; & \phantom{0}0.019 \;\pm\; & 0.013\,, \nonumber \\
& \AcpDkpipiKK          & \;=\;  \phantom{0}-0.045  \;\pm\; & \phantom{0}0.064 \;\pm\; & 0.011\,, \nonumber \\
& \AcpDkpipiPipi        & \;=\;  \phantom{0}-0.054  \;\pm\; & \phantom{0}0.101 \;\pm\; & 0.011\,, \nonumber \\
& \RpDkpipiKpi          & \;=\;  \phantom{-}0.0107  \;\pm\; & 0.0060 \;\pm\; & 0.0011\,, \nonumber \\
& \RmDkpipiKpi          & \;=\;  \phantom{-}0.0053  \;\pm\; & 0.0045 \;\pm\; & 0.0006\,, \nonumber
\end{alignat}


==> glwads-dkpipi-hh_stat.tex <==
\begin{tabular}{ l |cccccc}
\hline
                & \RcpDkpipi & \AfavDkpipiKpi & \AcpDkpipiKK & \AcpDkpipiPipi & \RpDkpipiKpi & \RmDkpipiKpi\\
\hline
\RcpDkpipi      &       1 &       0 &       0 &       0 &       0 &       0  \\
\AfavDkpipiKpi  &       0 &       1 &       0 &       0 &       0 &       0  \\
\AcpDkpipiKK    &       0 &       0 &       1 &   0.200 &       0 &       0  \\
\AcpDkpipiPipi  &       0 &       0 &   0.200 &       1 &       0 &       0  \\
\RpDkpipiKpi    &       0 &       0 &       0 &       0 &       1 &       0  \\
\RmDkpipiKpi    &       0 &       0 &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> glwads-dkpipi-hh_syst.tex <==
\begin{tabular}{ l |cccccc}
\hline
                & \RcpDkpipi & \AfavDkpipiKpi & \AcpDkpipiKK & \AcpDkpipiPipi & \RpDkpipiKpi & \RmDkpipiKpi\\
\hline
\RcpDkpipi      &       1 &       0 &       0 &       0 &       0 &       0  \\
\AfavDkpipiKpi  &       0 &       1 &       0 &       0 &       0 &       0  \\
\AcpDkpipiKK    &       0 &       0 &       1 &       0 &       0 &       0  \\
\AcpDkpipiPipi  &       0 &       0 &       0 &       1 &       0 &       0  \\
\RpDkpipiKpi    &       0 &       0 &       0 &       0 &       1 &       0  \\
\RmDkpipiKpi    &       0 &       0 &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> hfag_syst.tex <==
\begin{tabular}{ l |cccccc}
\hline
                & \xd & \yd & \ddKpi & \RdKpi & \DAcpPipi & \DAcpKK\\
\hline
\xd             &       1 &       0 &       0 &       0 &       0 &       0  \\
\yd             &       0 &       1 &       0 &       0 &       0 &       0  \\
\ddKpi          &       0 &       0 &       1 &       0 &       0 &       0  \\
\RdKpi          &       0 &       0 &       0 &       1 &       0 &       0  \\
\DAcpPipi       &       0 &       0 &       0 &       0 &       1 &       0  \\
\DAcpKK         &       0 &       0 &       0 &       0 &       0 &       1  \\
\hline
\end{tabular}


==> inputs_auxilary_old_format.tex <==
\section{Auxiliary inputs}
\label{sec:inputsauxilary}

A summary of all external inputs to the combination is provided in Table~\ref{tab:inputs_aux}.
These measurements provide constraints on the nuisance parameters which allows
for better precision on the value of \g.
The observable values
and the statistical and systematic uncertainties are described in Secs.~\ref{sec:input_hfag}-~\ref{sec:input_phis}.
The statistical and systematic correlations are provided in Appendix~\ref{sec:correlationsofinputs}.

\input{table-of-aux-inputs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[Charm system input from HFAG]{Input from global fit to charm data}
\label{sec:input_hfag}

The GLW/ADS measurements need input to constrain the charm
system in three areas: the ratio and string phase difference for \DzKpiFav and \DzKpiSup decays (\rdKpi, \ddKpi);
charm mixing (\xd, \yd); and direct \CP violation in \Dzhh decays
(\DAcpKK, \DAcpPipi). These are taken from a recent HFAG~\cite{Amhis:2014hma}
charm fit (CHARM 2015, ``Fit 3'', \CP violation allowed).
These do not include the latest results on $\Delta A_{CP}$ from LHCb~\cite{LHCb-PAPER-2015-055} but
their impact has been checked and found to be negligible.
The observables are
%
\input{results/hfag}
%
\noindent Here the value of \ddKpi was shifted by $\pi$ to comply with our phase convention.
The correlations of the charm parameters are given in Table~\ref{tab:hfagCor} in the Appendix.
The parameter \RdKpi is related to the amplitude ratio \rdKpi through
\begin{align}
	\label{eq:hfagrd}
	\RdKpi = \rdKpisq\,.
\end{align}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[The \DzKpipipi and \DzKpipiz CLEO-c and LHCb measurements]{\boldmath Input for \DzKpipipi and \DzKpipiz decays}
\label{sec:input_cleo}

The ADS measurements with \DzKpipiz and \DzKpipipi decays reach the best sensitivity when combined
with knowledge of the hadronic parameters describing the $D$ decays. These are the ratio, strong phase difference
and coherence factors of the two decays: \rdKpp, \ddKpp, \kdKpp and \rdKppp, \ddKppp, \kdKppp.
%In the previous combination \ddKppp and \kdKppp were constrained using a measurement published in~\cite{Libby:2014rea}.
%That likelihood was very non-Gaussian and was consequently taken directly as input into the \g combination.
%This was also done for \ddKpp and \kdKpp.
Recently an analysis of \DzKpipipi decays has been performed by LHCb~\cite{LHCb-PAPER-2015-057} that is sensitive to \rdKppp, \ddKppp and
\kdKppp. Furthermore, an updated measurement has been performed using CLEO-c data, and the results have been combined together with those from LHCb~\cite{Evans:2016tlp}
to yield contraints and correlations of the six relevant parameters; \rdKppp, \ddKppp, \kdKppp, \rdKpp, \ddKpp, \kdKpp.
These are included as Gaussian constraints in this combination. The effect of using the Gaussian constraints rather than the full
likelihood has been investigated and found to be negligible. The values used are
%
\input{results/cleo}
%
\noindent The correlation matrix is given in Table~\ref{tab:cleoCor} in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[$CP$ content of \Dhhpiz and \Dpipipipi]{\boldmath $CP$ content of \Dhhpiz and \Dpipipipi decays}

Important inputs to both the three body \Dhhpiz and four body \Dpipipipi quasi-GLW measurements are the fractional $CP$-even content of the decays, \FKKp, \Fppp, \Fpppp.
The values of these parameters are obtained from an analysis of \Dhhpiz and \Dpipipipi decays with data obtained by the CLEO-c experiment~\cite{Malde:2015mha}. The uncertainty for the $CP$-even content of \Dpipipipi decays is increased (from $\pm 0.028$) to account for the non-uniform acceptance of the LHCb detector as per the recommendation in Ref.~\cite{LHCb-PAPER-2016-003}. The values used are
%
\input{results/cleo_fcp}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[The \DKSKpi CLEO measurement]{\boldmath Input for \DKSKpi parameters}
\label{sec:input_cleo_glskskpi}

The \BuDh, \DKSKpi GLS measurement needs inputs for the charm system parameters
\rdKskpi, \ddKskpi, and \kdKskpi. They are constrained to the following values~\cite{Insler:2012pm}
\begin{align}
\RdKskpi         &=  0.356 \pm 0.034 \pm 0.007\,,\nonumber \\
\ddKskpi         &=  0.46 \pm 0.28\,,\nonumber \\
\kdKskpi         &=  1.00 \pm 0.16\,.\nonumber
\end{align}
In addition a measurement of the branching fraction ratio, \RdKskpi, from LHCb~\cite{LHCb-PAPER-2015-026} is used, which corresponds to a value of
\begin{align}
  \RdKskpi &= 0.370 \pm 0.003 \pm 0.012\,.\nonumber
\end{align}
The results correspond to
a limited region of the Dalitz plot dominated by the $K^{*}(892)^{+}$ resonance.
The quantity \RdKskpi is also related to \rdKskpi
through
\begin{equation}
\label{eq:rws_mixing_kskpi}
\RdKskpi = \rdKskpisq - \kdKskpi\rdKskpi(\yd\cos\ddKskpi-\xd\sin\ddKskpi) + \frac{1}{2}(\xd^2 + \yd^2)\,.
\end{equation}
%
The correlation between \ddKskpi and \kdKskpi is extracted from the experimental likelihood
as $\rho(\ddKskpi,\kdKskpi)=0.60$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[Constraints on the \BdDzKstz hadronic parameters]{\boldmath Constraints on the \BdDKstz hadronic parameters}
\label{sec:input_glwadsdkst_coherence}

The quasi-two-body \BdDKstz ADS and model-dependent GGSZ measurements need input on the coherence factor
\kbDKstz and the parameters $\RbDKstz = \rbDKstz / \rbDKpi$ and $\DbDKstz = \dbDKstz - \dbDKpi$, which relate the hadronic parameters of the quasi-two-body \BdDKstz ADS and GGSZ measurements
with those of the \BdDKpi amplitude analysis.
The resulting values are taken from the LHCb GLW-Dalitz analysis described in Ref.~\cite{LHCb-PAPER-2015-059}. They are
\begin{align}
\kbDKstz     &=  0.958 \pm 0.008 \pm 0.024, \nonumber\\
\RBDKstz     &=  1.020 \pm 0.020 \pm 0.060, \nonumber \\
\DBDKstz     &=  0.020 \pm 0.025 \pm 0.110, \nonumber
\end{align}
where the first uncertainty is statistical and the second systematic.
These are taken to be uncorrelated with each other and with the $x_{\pm}^{D\Kstarz}$,
$y_{\pm}^{D\Kstarz}$ parameters for the $\Bd\to\D\Kstarz$ decay that are determined
from the same analysis.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[Constraint on \phis]{\boldmath Constraint on \phis}
\label{sec:input_phis}

The time-dependent measurement of \BsDsK measures the quantity $\g-2\beta_s$.
In order to interpret this as a measurement of \g, the weak phase
$-2\beta_s$ is constrained to the measured value of \phis, taken from the LHCb
measurements of $\Bs\to\jpsi hh$~\cite{LHCb-PAPER-2014-059} decays to be
\begin{align}
\phis = -0.010 \pm 0.039 \rad\,. \nonumber
\end{align}


==> inputs_old_format.tex <==
\section{\boldmath Inputs from LHCb analyses sensitive to \g}
\label{sec:inputs}

The LHCb measurements used as inputs in the combination are summarised in Table~\ref{tab:inputs}. The observable values and the
statistical and systematic uncertainties are described in Secs.~\ref{sec:input_glwads}-~\ref{sec:input_dsk}. The statistical and systematic
correlations are provided in Appendix~\ref{sec:correlationsofinputs}. The observables are complementary between
methods and analyses, those labelled ``$D\pi$'' are only used in the \Dh combination.

\input{table-of-inputs}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BuDh, \Dhh GLW/ADS]{\boldmath\BuDh, \Dhh analysis}
\label{sec:input_glwads}

The GLW/ADS measurement using \BuDh, \Dzhh decays and the 3\invfb
data sample~\cite{LHCb-PAPER-2016-003} is an update of a previous analysis~\cite{LHCb-PAPER-2012-001}, which is included in the combination for the first time.
The observables are defined in analogy to Eqs.~(\ref{eq:af}-\ref{eq:aads}), and the measured values are,
%
\input{results/dh/glwads-dh-hh}
%
\noindent where the first uncertainty is statistical and the second is systematic. For \RCPKK and \RCPPiPi the third
uncertainty arises from the assumption that $\rbpi=0$ as discussed in Ref.~\cite{LHCb-PAPER-2016-003} and subsequently applies
only for the \robust combination.
Their statistical and systematic correlations are given in Tables~\ref{tab:glwadshhCor}
and~\ref{tab:glwadshhCorSyst} in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BuDh, \Dzhpipipi quasi-GLW/ADS]{\boldmath\BuDh, \Dhpipipi analysis}
\label{sec:input_adsk3pi}

The ADS measurement using the \BuDh, \DKpipipi decay mode and 3\invfb of
data~\cite{LHCb-PAPER-2016-003} is an update of a previous measurement~\cite{LHCb-PAPER-2012-055}.
The method to use these decays to constrain \g is described in Ref.~\cite{Nayak:2014tea}.
The quasi-GLW measurement with \BuDh, \Dpipipipi decays is included in the combination for the first time.
The label ``quasi'' is used because the \Dpipipipi decay is not completely \CP-even, the fraction of \CP-even content is given by \Fpppp as described in Sec.~\ref{sec:inputsauxilary}.
The observables are defined in analogy to Eqs.~(\ref{eq:af}--\ref{eq:rads}),
and the measured values are
%
\input{results/dh/glwads-dh-h3pi}
%
\noindent where the first uncertainty is statistical and the second is systematic. The third uncertainty for \RCPpppp
is again from the assumption that $\rbpi=0$ and subsequently applies only for the \robust combination.
Their statistical and systematic correlations are given in Tables~\ref{tab:glwadsk3piCor} and~\ref{tab:glwadsk3piCorSyst} in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BuDh, \Dhhpiz quasi-GLW/ADS]{\boldmath\BuDh, \Dhhpiz analysis}
\label{sec:input_adskpipiz}

Inputs from the quasi-GLW/ADS analysis of \BuDh, \Dhhpiz decays using 3\invfb of
data~\cite{LHCb-PAPER-2015-014} are new to this combination.
The \CP-even content of the \DKKpiz (\Dpipipiz) decay mode is given by the parameter \FKKp (\Fppp), as described in Sec.~\ref{sec:inputsauxilary}.
The observables are defined in analogy to Eqs.~(\ref{eq:af}--\ref{eq:rads}),
and the measured values are
%
\input{results/dh/glwads-dh-hhpi0}
%
\noindent where the first uncertainty is statistical and the second is systematic.
The statistical and systematic correlations are given in Tables~\ref{tab:glwadshhpizCor}
and~\ref{tab:glwadshhpizCorSyst} in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BuDK, \DKShh GGSZ]{\boldmath\BuDK, \DKShh analysis}
\label{sec:input_ggsz}

The inputs from the model-independent GGSZ~\cite{Bondar:2001vn,Giri:2003ty} analysis
of \BuDK, \DKShh decays, which uses 3\invfb of data~\cite{LHCb-PAPER-2014-041}, are the same as those used in the previous combination~\cite{LHCb-CONF-2014-004}.
The variables $\xpm = \rb\cos(\db\pm\g)$ and $\ypm = \rb\sin(\db\pm\g)$ are obtained from a fit
to the Dalitz plane of $\DKSpipi$ and $\DKSKK$ decays.
The results are
%
\input{results/ggsz-dk}
%
\noindent where the first uncertainty is statistical, the second is systematic, and the third is an external uncertainty due to the information on the
strong phase variation across the \DKShh phase space. Correlations between the statistical and systematic uncertainties are given in Tables~\ref{tab:ggszCor}
and~\ref{tab:ggszCorSyst} in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BuDK, \DKSKpi GLS]{\boldmath\BuDh, \DKSKpi analysis}
\label{sec:input_glskskpi}

The inputs from the GLS analysis
of \BuDh, \DKSKpi decays~\cite{LHCb-PAPER-2013-068}, which uses the 3\invfb data sample,
are the same as those included in the last combination~\cite{LHCb-CONF-2014-004}.
The observables are defined in analogy to Eqs.~(\ref{eq:af}, \ref{eq:rads}--\ref{eq:aads})
and are measured to be
%
\input{results/gls}
%
\noindent where the first uncertainty is statistical and the second is systematic.
These values correspond to the restricted ``$K^{*}(892)^{+}$'' region of the
\DKSKpi phase space, as they offer better sensitivity to \g: the
two-dimensional \g--\rb confidence region computed in Ref.~\cite{LHCb-PAPER-2013-068}
is smaller than for the full phase space.
The statistical and systematic correlations are given in Tables~\ref{tab:glsCor} and~\ref{tab:glsCorSyst} in the Appendix.

Input from \BuDpi with \DKSKpi decays is not used because the correction for \CP violation and mixing in the neutral kaon
system is expected to be $\mathcal{O}(1)$ for $\rbpi\approx 0.005$.
%
%For the \robust combination, the ratios are combined in order to
%cancel any information coming from the \BuDpi system,
%\begin{align}
%\RfavsupDkKskpi = \frac{\RfavDkDpiKskpi}{\RsupDkDpiKskpi} \cdot \RfavsupDpiKskpi\,,
%\end{align}
%which is computed, taking correlations
%into account, to be
%\begin{align}
%\RfavsupDkKskpi = 3.86  \pm 0.94\stat \pm 0.21\syst\,.
%\end{align}{\bf can we avoid the above discussion and just give the value?}
%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BuDhpipi, \Dzhh GLW/ADS]{\boldmath\BuDhpipi, \Dhh analysis}
\label{sec:input_glwadsdkpipi}

The inputs from the LHCb GLW/ADS analysis of \BuDhpipi, \Dzhh decays~\cite{LHCb-PAPER-2015-020}, which uses 3\invfb of data,
are included in the combination for the first time.
The observables are defined in analogy to Eqs.~(\ref{eq:rcp},\ref{eq:af},\ref{eq:rp}-
ref{eq:rm}) and are found to be
%
\input{results/dh/glwads-dhpipi-hh}
%
\noindent where the first uncertainty is statistical and the second is systematic. For \RcpDkpipi, the single uncertainty includes both statistical and systematic contributions.
The correlations are given in Tables~\ref{tab:glwadsdkpipiCor}
and~\ref{tab:glwadsdkpipiCorSyst} in the Appendix.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BdDzKstz, \DzKpi ADS]{\boldmath\BdDzKstz, \DKpi analysis}
\label{sec:input_glwadsdkst}

The inputs from the ADS analysis
of \BdDzKstz, \DzKpi decays using 3\invfb of data~\cite{LHCb-PAPER-2014-028}
are included as they were in the previous combination~\cite{LHCb-CONF-2014-004}. However, the GLW part of this
analysis (with \DzKK and \Dzpipi) has been superseded by the Dalitz plot analysis described in Sec.~\ref{sec:input_dalitzdkst}.
The ADS observables are defined in analogy to Eqs.~(\ref{eq:af},\ref{eq:rp}-\ref{eq:rm}) and the measured values are,
%
\input{results/ads-dkstz}
%
\noindent where the first uncertainty is statistical and the second is systematic.
The statistical correlations are given in Table~\ref{tab:glwadsdkstCor},
and the systematic correlations in Table~\ref{tab:glwadsdkstCorSyst}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BdDKpi, \Dzhh GLW-Dalitz]{\boldmath\BdDKpi, \Dhh analysis}
\label{sec:input_dalitzdkst}

Information from the GLW-Dalitz analysis of \BdDKpi, \Dzhh decays performed using 3\invfb~\cite{LHCb-PAPER-2015-059}
is added to the combination for the first time.
The ``Dalitz'' label is used to indicate the method used to extract information about \CP violation in this mode.
The variables $\xpm^{DK\pi} = \rbDKpi\cos(\dbDKpi\pm\g)$ and $\ypm^{DK\pi} = \rbDKpi\sin(\dbDKpi\pm\g)$ are determined, from a simultaneous Dalitz
plot fit to $\Dz\to\Km\pip$, $D\to\Kp\Km$ and $D\to\pip\pim$ samples, as described in Refs.~\cite{Gershon:2008pe,Gershon:2009qc}.
The results are
%
\input{results/glw-dalitz-dkstz}
%
\noindent where the first uncertainty is statistical and the second is systematic.
The correlations are given in Tables~\ref{tab:glwkstCor} and~\ref{tab:glwkstCorSyst} in the Appendix.
Constraints on hadronic parameters are also obtained in this analysis, as described in Sec.~\ref{sec:input_glwadsdkst_coherence}.

%The analysis also provides measurements to enable the combination of \BdDKpi and \BdDzKstz results.
%The coherence factor is determined to be
%\begin{align}
%\kbDKstz &= ...,
%\end{align}
%where the first uncertainty is statistical and the second is systematic.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BdDzKstz, \DKSpipi GGSZ]{\boldmath\BdDzKstz, \DKSpipi analysis}
\label{sec:input_ggszdkst}

Inputs from the model-dependent GGSZ analysis of \BdDzKstz, \DKSpipi decays using 3\invfb of data~\cite{LHCb-PAPER-2016-007}
are included in the combination for the first time.
The observables $\xpm^{D\Kstarz} = \rbDKstz\cos(\dbDKstz\pm\g)$ and $\ypm^{D\Kstarz} = \rbDKstz\sin(\dbDKstz\pm\g)$ are measured by fitting
the $\DKSpipi$ Dalitz plot using a model from BaBar~\cite{delAmoSanchez:2010xz}.
The results are
%
\input{results/ggsz-dkstz}
%
\noindent where the first uncertainty is statistical, the second is systematic and the third is from the Dalitz plot fit model.
The correlations are given in Tables~\ref{tab:ggszkstCor}
and~\ref{tab:ggszkstCorSyst} in the Appendix.

A model-independent GGSZ analysis~\cite{LHCb-PAPER-2016-006} is also performed by LHCb on the same data sample. Currently, the model-dependent analysis
has the best sensitivity to the parameters $\xpm$ and $\ypm$. Therefore the model-dependent results
are used in the combination.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection[\BsDsK time dependent]{\boldmath\BsDsK analysis}
\label{sec:input_dsk}

The inputs used from the time-dependent analysis
of \BsDsK decays
using 1\invfb of data~\cite{LHCb-PAPER-2014-038}
are identical to those used in Ref.~\cite{LHCb-CONF-2014-004}.
The results for the observables are
\input{results/dsk}
\noindent where the first uncertainty is statistical and the second is systematic.
The statistical correlations are given in Table~\ref{tab:dskCor},
and the systematic correlations in Table~\ref{tab:dskCorSyst} in the
Appendix.


==> layout.tex <==
\section{Layout}

\begin{enumerate}

\item Unnecessary blank space should be avoided, between paragraphs or
  around figures and tables.

\item Figure and table captions should be concise and use a somewhat smaller typeface
  than the main text, to help distinguish them. This is achieved by 
  inserting \verb!\small! at the beginning of the caption.
  (NB with the latest version of the file \verb!premable.tex! this is automatic)
  Figure captions go below the figure, table captions go above the
  table.

\item Captions and footnotes should be punctuated correctly, like
  normal text. The use of too many footnotes should be avoided:
  typically they are used for giving commercial details of companies,
  or standard items like coordinate system definition or the implicit
  inclusion of charge-conjugate processes.\footnote{If placed at the end
    of a sentence, the footnote symbol normally follows the
    punctuation; if placed in the middle of an equation, take care to
    avoid any possible confusion with an index.}$^,$\footnote{The standard footnote reads: ``The inclusion of charge-conjugate processes is implied
    throughout.'' This may need to be modified, for example with ``except in the discussion of asymmetries.''}

\item Tables should be formatted in a simple fashion, without
  excessive use of horizontal and vertical lines. See
  Table~\ref{tab:example} for an example.

\item Figures and tables should normally be placed so that they appear
  on the same page as their first reference, but at the top or bottom
  of the page; if this is not possible, they should come as soon as
  possible afterwards.  They must all be referred to from the text.

\item If one or more equations are referenced, all equations should be numbered using parentheses as shown in
  Eq.~\ref{eq:CKM},
  \begin{equation}
    \label{eq:CKM}
    V_{\uquark\squark}V_{\uquark\bquark}^* + 
    V_{\cquark\squark}V_{\cquark\bquark}^* + 
    V_{\tquark\squark}V_{\tquark\bquark}^* = 0 \ . 
  \end{equation}
  
\item Displayed results like
  \begin{equation*}
    \BF(\decay{\Bs}{\mumu}) < 1.5 \times 10^{-8} \text{ at 95\% CL}
  \end{equation*}
  should in general not be numbered.

\item Numbered equations should be avoided in captions and footnotes.

\item Displayed equations are part of the normal grammar of the
  text. This means that the equation should end in full stop or comma if
  required when reading aloud. The line after the equation should only
  be indented if it starts a new paragraph.

\item Sub-sectioning should not be excessive: sections with more than three
levels of index (1.1.1) should be avoided.

%\item It is generally preferable to itemize a list using numbers rather
%than bullets.

\item Acronyms should be defined the first time they are used,
  \eg ``Monte Carlo~(MC) events containing a doubly
  Cabibbo-suppressed~(DCS) decay have been generated.''
  The abbreviated words should not be capitalised if it is not naturally
  written with capitals, \eg quantum chromodynamics (QCD),
  impact parameter (IP), boosted decision tree (BDT).
  Avoid acronyms if they are used three times or less.
  A sentence should never start with an acronym and its better to
  avoid it as the last word of a sentence as well.

\end{enumerate}

\begin{table}[t]
  \caption{
    %\small %captions should be a little bit smaller than main text
    Background-to-signal ratio estimated in a $\pm 50\mevcc$ 
    mass window for the prompt and long-lived backgrounds, and the 
    minimum bias rate.}
\begin{center}\begin{tabular}{lccc}
    \hline
    Channel                           & $B_{\mathrm{pr}}/S$ & $B_{\mathrm{LL}}/S$   & MB rate       \\ 
    \hline
    \BsToJPsiPhi              & $ 1.6 \pm 0.6$ & $ 0.51 \pm 0.08$ & $\sim 0.3$ Hz \\
    \BdToJPsiKst              & $ 5.2 \pm 0.3$ & $1.53 \pm 0.08 $ & $\sim 8.1$ Hz \\
    \decay{\Bp}{\jpsi\Kstarp} & $ 1.6 \pm 0.2$ & $0.29 \pm 0.06$  & $\sim 1.4$ Hz \\
    \hline
  \end{tabular}\end{center}
\label{tab:example}
\end{table}

% old table with vertical lines
%\begin{table}[t]
%  \caption{
%    \small %captions should be a little bit smaller than main text
%    Background-to-signal ratio estimated in a $\pm 50\mevcc$ 
%    mass window for the prompt and long-lived backgrounds, and the 
%    minimum bias rate.}
%\begin{center}\begin{tabular}{l|c|c|c}
%    Channel                           & $B_{\mathrm{pr}}}/S$ & $B_{{\mathrm{LL}}/S$   & MB rate       \\ 
%    \hline
%    \BsToJPsiPhi              & $ 1.6 \pm 0.6$ & $ 0.51 \pm 0.08$ & $\sim 0.3$ Hz \\
%    \BdToJPsiKst              & $ 5.2 \pm 0.3$ & $1.53 \pm 0.08 $ & $\sim 8.1$ Hz \\
%    \decay{\Bp}{\jpsi\Kstarp} & $ 1.6 \pm 0.2$ & $0.29 \pm 0.06$  & $\sim 1.4$ Hz \\
%  \end{tabular}\end{center}
%\label{tab:example}
%\end{table}


==> lhcb-symbols-list.tex <==
% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\section{List of all symbols}
\label{sec:listofsymbols}
\subsection{Experiments}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash lhcb} & \lhcb & \texttt{\textbackslash atlas} & \atlas & \texttt{\textbackslash cms} & \cms \\
\texttt{\textbackslash alice} & \alice & \texttt{\textbackslash babar} & \babar & \texttt{\textbackslash belle} & \belle \\
\texttt{\textbackslash cleo} & \cleo & \texttt{\textbackslash cdf} & \cdf & \texttt{\textbackslash dzero} & \dzero \\
\texttt{\textbackslash aleph} & \aleph & \texttt{\textbackslash delphi} & \delphi & \texttt{\textbackslash opal} & \opal \\
\texttt{\textbackslash lthree} & \lthree & \texttt{\textbackslash sld} & \sld & \texttt{\textbackslash cern} & \cern \\
\texttt{\textbackslash lhc} & \lhc & \texttt{\textbackslash lep} & \lep & \texttt{\textbackslash tevatron} & \tevatron \\
\end{tabular*}

\subsubsection{LHCb sub-detectors and sub-systems}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash velo} & \velo & \texttt{\textbackslash rich} & \rich & \texttt{\textbackslash richone} & \richone \\
\texttt{\textbackslash richtwo} & \richtwo & \texttt{\textbackslash ttracker} & \ttracker & \texttt{\textbackslash intr} & \intr \\
\texttt{\textbackslash st} & \st & \texttt{\textbackslash ot} & \ot & \texttt{\textbackslash spd} & \spd \\
\texttt{\textbackslash presh} & \presh & \texttt{\textbackslash ecal} & \ecal & \texttt{\textbackslash hcal} & \hcal \\
\texttt{\textbackslash MagUp} & \MagUp & \texttt{\textbackslash MagDown} & \MagDown & \texttt{\textbackslash ode} & \ode \\
\texttt{\textbackslash daq} & \daq & \texttt{\textbackslash tfc} & \tfc & \texttt{\textbackslash ecs} & \ecs \\
\texttt{\textbackslash lone} & \lone & \texttt{\textbackslash hlt} & \hlt & \texttt{\textbackslash hltone} & \hltone \\
\texttt{\textbackslash hlttwo} & \hlttwo &  \\
\end{tabular*}

\subsection{Particles}
\subsubsection{Leptons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash electron} & \electron & \texttt{\textbackslash en} & \en & \texttt{\textbackslash ep} & \ep \\
\texttt{\textbackslash epm} & \epm & \texttt{\textbackslash epem} & \epem & \texttt{\textbackslash muon} & \muon \\
\texttt{\textbackslash mup} & \mup & \texttt{\textbackslash mun} & \mun & \texttt{\textbackslash mumu} & \mumu \\
\texttt{\textbackslash tauon} & \tauon & \texttt{\textbackslash taup} & \taup & \texttt{\textbackslash taum} & \taum \\
\texttt{\textbackslash tautau} & \tautau & \texttt{\textbackslash lepton} & \lepton & \texttt{\textbackslash ellm} & \ellm \\
\texttt{\textbackslash ellp} & \ellp & \texttt{\textbackslash ellell} & \ellell & \texttt{\textbackslash neu} & \neu \\
\texttt{\textbackslash neub} & \neub & \texttt{\textbackslash neue} & \neue & \texttt{\textbackslash neueb} & \neueb \\
\texttt{\textbackslash neum} & \neum & \texttt{\textbackslash neumb} & \neumb & \texttt{\textbackslash neut} & \neut \\
\texttt{\textbackslash neutb} & \neutb & \texttt{\textbackslash neul} & \neul & \texttt{\textbackslash neulb} & \neulb \\
\end{tabular*}

\subsubsection{Gauge bosons and scalars}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash g} & \g & \texttt{\textbackslash H} & \H & \texttt{\textbackslash Hp} & \Hp \\
\texttt{\textbackslash Hm} & \Hm & \texttt{\textbackslash Hpm} & \Hpm & \texttt{\textbackslash W} & \W \\
\texttt{\textbackslash Wp} & \Wp & \texttt{\textbackslash Wm} & \Wm & \texttt{\textbackslash Wpm} & \Wpm \\
\texttt{\textbackslash Z} & \Z &  \\
\end{tabular*}

\subsubsection{Quarks}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash quark} & \quark & \texttt{\textbackslash quarkbar} & \quarkbar & \texttt{\textbackslash qqbar} & \qqbar \\
\texttt{\textbackslash uquark} & \uquark & \texttt{\textbackslash uquarkbar} & \uquarkbar & \texttt{\textbackslash uubar} & \uubar \\
\texttt{\textbackslash dquark} & \dquark & \texttt{\textbackslash dquarkbar} & \dquarkbar & \texttt{\textbackslash ddbar} & \ddbar \\
\texttt{\textbackslash squark} & \squark & \texttt{\textbackslash squarkbar} & \squarkbar & \texttt{\textbackslash ssbar} & \ssbar \\
\texttt{\textbackslash cquark} & \cquark & \texttt{\textbackslash cquarkbar} & \cquarkbar & \texttt{\textbackslash ccbar} & \ccbar \\
\texttt{\textbackslash bquark} & \bquark & \texttt{\textbackslash bquarkbar} & \bquarkbar & \texttt{\textbackslash bbbar} & \bbbar \\
\texttt{\textbackslash tquark} & \tquark & \texttt{\textbackslash tquarkbar} & \tquarkbar & \texttt{\textbackslash ttbar} & \ttbar \\
\end{tabular*}

\subsubsection{Light mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash hadron} & \hadron & \texttt{\textbackslash pion} & \pion & \texttt{\textbackslash piz} & \piz \\
\texttt{\textbackslash pizs} & \pizs & \texttt{\textbackslash pip} & \pip & \texttt{\textbackslash pim} & \pim \\
\texttt{\textbackslash pipm} & \pipm & \texttt{\textbackslash pimp} & \pimp & \texttt{\textbackslash rhomeson} & \rhomeson \\
\texttt{\textbackslash rhoz} & \rhoz & \texttt{\textbackslash rhop} & \rhop & \texttt{\textbackslash rhom} & \rhom \\
\texttt{\textbackslash rhopm} & \rhopm & \texttt{\textbackslash rhomp} & \rhomp & \texttt{\textbackslash kaon} & \kaon \\
\texttt{\textbackslash Kb} & \Kb & \texttt{\textbackslash KorKbar} & \KorKbar & \texttt{\textbackslash Kz} & \Kz \\
\texttt{\textbackslash Kzb} & \Kzb & \texttt{\textbackslash Kp} & \Kp & \texttt{\textbackslash Km} & \Km \\
\texttt{\textbackslash Kpm} & \Kpm & \texttt{\textbackslash Kmp} & \Kmp & \texttt{\textbackslash KS} & \KS \\
\texttt{\textbackslash KL} & \KL & \texttt{\textbackslash Kstarz} & \Kstarz & \texttt{\textbackslash Kstarzb} & \Kstarzb \\
\texttt{\textbackslash Kstar} & \Kstar & \texttt{\textbackslash Kstarb} & \Kstarb & \texttt{\textbackslash Kstarp} & \Kstarp \\
\texttt{\textbackslash Kstarm} & \Kstarm & \texttt{\textbackslash Kstarpm} & \Kstarpm & \texttt{\textbackslash Kstarmp} & \Kstarmp \\
\texttt{\textbackslash etaz} & \etaz & \texttt{\textbackslash etapr} & \etapr & \texttt{\textbackslash phiz} & \phiz \\
\texttt{\textbackslash omegaz} & \omegaz &  \\
\end{tabular*}

\subsubsection{Heavy mesons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash D} & \D & \texttt{\textbackslash Db} & \Db & \texttt{\textbackslash DorDbar} & \DorDbar \\
\texttt{\textbackslash Dz} & \Dz & \texttt{\textbackslash Dzb} & \Dzb & \texttt{\textbackslash Dp} & \Dp \\
\texttt{\textbackslash Dm} & \Dm & \texttt{\textbackslash Dpm} & \Dpm & \texttt{\textbackslash Dmp} & \Dmp \\
\texttt{\textbackslash Dstar} & \Dstar & \texttt{\textbackslash Dstarb} & \Dstarb & \texttt{\textbackslash Dstarz} & \Dstarz \\
\texttt{\textbackslash Dstarzb} & \Dstarzb & \texttt{\textbackslash Dstarp} & \Dstarp & \texttt{\textbackslash Dstarm} & \Dstarm \\
\texttt{\textbackslash Dstarpm} & \Dstarpm & \texttt{\textbackslash Dstarmp} & \Dstarmp & \texttt{\textbackslash Ds} & \Ds \\
\texttt{\textbackslash Dsp} & \Dsp & \texttt{\textbackslash Dsm} & \Dsm & \texttt{\textbackslash Dspm} & \Dspm \\
\texttt{\textbackslash Dsmp} & \Dsmp & \texttt{\textbackslash Dss} & \Dss & \texttt{\textbackslash Dssp} & \Dssp \\
\texttt{\textbackslash Dssm} & \Dssm & \texttt{\textbackslash Dsspm} & \Dsspm & \texttt{\textbackslash Dssmp} & \Dssmp \\
\texttt{\textbackslash B} & \B & \texttt{\textbackslash Bbar} & \Bbar & \texttt{\textbackslash Bb} & \Bb \\
\texttt{\textbackslash BorBbar} & \BorBbar & \texttt{\textbackslash Bz} & \Bz & \texttt{\textbackslash Bzb} & \Bzb \\
\texttt{\textbackslash Bu} & \Bu & \texttt{\textbackslash Bub} & \Bub & \texttt{\textbackslash Bp} & \Bp \\
\texttt{\textbackslash Bm} & \Bm & \texttt{\textbackslash Bpm} & \Bpm & \texttt{\textbackslash Bmp} & \Bmp \\
\texttt{\textbackslash Bd} & \Bd & \texttt{\textbackslash Bs} & \Bs & \texttt{\textbackslash Bsb} & \Bsb \\
\texttt{\textbackslash Bdb} & \Bdb & \texttt{\textbackslash Bc} & \Bc & \texttt{\textbackslash Bcp} & \Bcp \\
\texttt{\textbackslash Bcm} & \Bcm & \texttt{\textbackslash Bcpm} & \Bcpm &  \\
\end{tabular*}

\subsubsection{Onia}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash jpsi} & \jpsi & \texttt{\textbackslash psitwos} & \psitwos & \texttt{\textbackslash psiprpr} & \psiprpr \\
\texttt{\textbackslash etac} & \etac & \texttt{\textbackslash chiczero} & \chiczero & \texttt{\textbackslash chicone} & \chicone \\
\texttt{\textbackslash chictwo} & \chictwo & \texttt{\textbackslash OneS} & \OneS & \texttt{\textbackslash TwoS} & \TwoS \\
\texttt{\textbackslash ThreeS} & \ThreeS & \texttt{\textbackslash FourS} & \FourS & \texttt{\textbackslash FiveS} & \FiveS \\
\texttt{\textbackslash chic} & \chic &  \\
\end{tabular*}

\subsubsection{Baryons}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash proton} & \proton & \texttt{\textbackslash antiproton} & \antiproton & \texttt{\textbackslash neutron} & \neutron \\
\texttt{\textbackslash antineutron} & \antineutron & \texttt{\textbackslash Deltares} & \Deltares & \texttt{\textbackslash Deltaresbar} & \Deltaresbar \\
\texttt{\textbackslash Xires} & \Xires & \texttt{\textbackslash Xiresbar} & \Xiresbar & \texttt{\textbackslash Lz} & \Lz \\
\texttt{\textbackslash Lbar} & \Lbar & \texttt{\textbackslash LorLbar} & \LorLbar & \texttt{\textbackslash Lambdares} & \Lambdares \\
\texttt{\textbackslash Lambdaresbar} & \Lambdaresbar & \texttt{\textbackslash Sigmares} & \Sigmares & \texttt{\textbackslash Sigmaresbar} & \Sigmaresbar \\
\texttt{\textbackslash Omegares} & \Omegares & \texttt{\textbackslash Omegaresbar} & \Omegaresbar & \texttt{\textbackslash Lb} & \Lb \\
\texttt{\textbackslash Lbbar} & \Lbbar & \texttt{\textbackslash Lc} & \Lc & \texttt{\textbackslash Lcbar} & \Lcbar \\
\texttt{\textbackslash Xib} & \Xib & \texttt{\textbackslash Xibz} & \Xibz & \texttt{\textbackslash Xibm} & \Xibm \\
\texttt{\textbackslash Xibbar} & \Xibbar & \texttt{\textbackslash Xibbarz} & \Xibbarz & \texttt{\textbackslash Xibbarp} & \Xibbarp \\
\texttt{\textbackslash Xic} & \Xic & \texttt{\textbackslash Xicz} & \Xicz & \texttt{\textbackslash Xicp} & \Xicp \\
\texttt{\textbackslash Xicbar} & \Xicbar & \texttt{\textbackslash Xicbarz} & \Xicbarz & \texttt{\textbackslash Xicbarm} & \Xicbarm \\
\texttt{\textbackslash Omegac} & \Omegac & \texttt{\textbackslash Omegacbar} & \Omegacbar & \texttt{\textbackslash Omegab} & \Omegab \\
\texttt{\textbackslash Omegabbar} & \Omegabbar &  \\
\end{tabular*}

\subsection{Physics symbols}
\subsubsection{Decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BF} & \BF & \texttt{\textbackslash BRvis} & \BRvis & \texttt{\textbackslash BR} & \BR \\
\texttt{\textbackslash decay[2] \textbackslash decay\{\Pa\}\{\Pb \Pc\}} & \decay{\Pa}{\Pb \Pc} & \texttt{\textbackslash ra} & \ra & \texttt{\textbackslash to} & \to \\
\end{tabular*}

\subsubsection{Lifetimes}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tauBs} & \tauBs & \texttt{\textbackslash tauBd} & \tauBd & \texttt{\textbackslash tauBz} & \tauBz \\
\texttt{\textbackslash tauBu} & \tauBu & \texttt{\textbackslash tauDp} & \tauDp & \texttt{\textbackslash tauDz} & \tauDz \\
\texttt{\textbackslash tauL} & \tauL & \texttt{\textbackslash tauH} & \tauH &  \\
\end{tabular*}

\subsubsection{Masses}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash mBd} & \mBd & \texttt{\textbackslash mBp} & \mBp & \texttt{\textbackslash mBs} & \mBs \\
\texttt{\textbackslash mBc} & \mBc & \texttt{\textbackslash mLb} & \mLb &  \\
\end{tabular*}

\subsubsection{EW theory, groups}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash grpsuthree} & \grpsuthree & \texttt{\textbackslash grpsutw} & \grpsutw & \texttt{\textbackslash grpuone} & \grpuone \\
\texttt{\textbackslash ssqtw} & \ssqtw & \texttt{\textbackslash csqtw} & \csqtw & \texttt{\textbackslash stw} & \stw \\
\texttt{\textbackslash ctw} & \ctw & \texttt{\textbackslash ssqtwef} & \ssqtwef & \texttt{\textbackslash csqtwef} & \csqtwef \\
\texttt{\textbackslash stwef} & \stwef & \texttt{\textbackslash ctwef} & \ctwef & \texttt{\textbackslash gv} & \gv \\
\texttt{\textbackslash ga} & \ga & \texttt{\textbackslash order} & \order & \texttt{\textbackslash ordalph} & \ordalph \\
\texttt{\textbackslash ordalsq} & \ordalsq & \texttt{\textbackslash ordalcb} & \ordalcb &  \\
\end{tabular*}

\subsubsection{QCD parameters}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash as} & \as & \texttt{\textbackslash MSb} & \MSb & \texttt{\textbackslash lqcd} & \lqcd \\
\texttt{\textbackslash qsq} & \qsq &  \\
\end{tabular*}

\subsubsection{CKM, CP violation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eps} & \eps & \texttt{\textbackslash epsK} & \epsK & \texttt{\textbackslash epsB} & \epsB \\
\texttt{\textbackslash epsp} & \epsp & \texttt{\textbackslash CP} & \CP & \texttt{\textbackslash CPT} & \CPT \\
\texttt{\textbackslash rhobar} & \rhobar & \texttt{\textbackslash etabar} & \etabar & \texttt{\textbackslash Vud} & \Vud \\
\texttt{\textbackslash Vcd} & \Vcd & \texttt{\textbackslash Vtd} & \Vtd & \texttt{\textbackslash Vus} & \Vus \\
\texttt{\textbackslash Vcs} & \Vcs & \texttt{\textbackslash Vts} & \Vts & \texttt{\textbackslash Vub} & \Vub \\
\texttt{\textbackslash Vcb} & \Vcb & \texttt{\textbackslash Vtb} & \Vtb & \texttt{\textbackslash Vuds} & \Vuds \\
\texttt{\textbackslash Vcds} & \Vcds & \texttt{\textbackslash Vtds} & \Vtds & \texttt{\textbackslash Vuss} & \Vuss \\
\texttt{\textbackslash Vcss} & \Vcss & \texttt{\textbackslash Vtss} & \Vtss & \texttt{\textbackslash Vubs} & \Vubs \\
\texttt{\textbackslash Vcbs} & \Vcbs & \texttt{\textbackslash Vtbs} & \Vtbs &  \\
\end{tabular*}

\subsubsection{Oscillations}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dm} & \dm & \texttt{\textbackslash dms} & \dms & \texttt{\textbackslash dmd} & \dmd \\
\texttt{\textbackslash DG} & \DG & \texttt{\textbackslash DGs} & \DGs & \texttt{\textbackslash DGd} & \DGd \\
\texttt{\textbackslash Gs} & \Gs & \texttt{\textbackslash Gd} & \Gd & \texttt{\textbackslash MBq} & \MBq \\
\texttt{\textbackslash DGq} & \DGq & \texttt{\textbackslash Gq} & \Gq & \texttt{\textbackslash dmq} & \dmq \\
\texttt{\textbackslash GL} & \GL & \texttt{\textbackslash GH} & \GH & \texttt{\textbackslash DGsGs} & \DGsGs \\
\texttt{\textbackslash Delm} & \Delm & \texttt{\textbackslash ACP} & \ACP & \texttt{\textbackslash Adir} & \Adir \\
\texttt{\textbackslash Amix} & \Amix & \texttt{\textbackslash ADelta} & \ADelta & \texttt{\textbackslash phid} & \phid \\
\texttt{\textbackslash sinphid} & \sinphid & \texttt{\textbackslash phis} & \phis & \texttt{\textbackslash betas} & \betas \\
\texttt{\textbackslash sbetas} & \sbetas & \texttt{\textbackslash stbetas} & \stbetas & \texttt{\textbackslash stphis} & \stphis \\
\texttt{\textbackslash sinphis} & \sinphis &  \\
\end{tabular*}

\subsubsection{Tagging}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash edet} & \edet & \texttt{\textbackslash erec} & \erec & \texttt{\textbackslash esel} & \esel \\
\texttt{\textbackslash etrg} & \etrg & \texttt{\textbackslash etot} & \etot & \texttt{\textbackslash mistag} & \mistag \\
\texttt{\textbackslash wcomb} & \wcomb & \texttt{\textbackslash etag} & \etag & \texttt{\textbackslash etagcomb} & \etagcomb \\
\texttt{\textbackslash effeff} & \effeff & \texttt{\textbackslash effeffcomb} & \effeffcomb & \texttt{\textbackslash efftag} & \efftag \\
\texttt{\textbackslash effD} & \effD & \texttt{\textbackslash etagprompt} & \etagprompt & \texttt{\textbackslash etagLL} & \etagLL \\
\end{tabular*}

\subsubsection{Key decay channels}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdToKstmm} & \BdToKstmm & \texttt{\textbackslash BdbToKstmm} & \BdbToKstmm & \texttt{\textbackslash BsToJPsiPhi} & \BsToJPsiPhi \\
\texttt{\textbackslash BdToJPsiKst} & \BdToJPsiKst & \texttt{\textbackslash BdbToJPsiKst} & \BdbToJPsiKst & \texttt{\textbackslash BsPhiGam} & \BsPhiGam \\
\texttt{\textbackslash BdKstGam} & \BdKstGam & \texttt{\textbackslash BTohh} & \BTohh & \texttt{\textbackslash BdTopipi} & \BdTopipi \\
\texttt{\textbackslash BdToKpi} & \BdToKpi & \texttt{\textbackslash BsToKK} & \BsToKK & \texttt{\textbackslash BsTopiK} & \BsTopiK \\
\end{tabular*}

\subsubsection{Rare decays}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash BdKstee} & \BdKstee & \texttt{\textbackslash BdbKstee} & \BdbKstee & \texttt{\textbackslash bsll} & \bsll \\
\texttt{\textbackslash AFB} & \AFB & \texttt{\textbackslash FL} & \FL & \texttt{\textbackslash AT\#1 \textbackslash AT2} & \AT2 \\
\texttt{\textbackslash btosgam} & \btosgam & \texttt{\textbackslash btodgam} & \btodgam & \texttt{\textbackslash Bsmm} & \Bsmm \\
\texttt{\textbackslash Bdmm} & \Bdmm & \texttt{\textbackslash ctl} & \ctl & \texttt{\textbackslash ctk} & \ctk \\
\end{tabular*}

\subsubsection{Wilson coefficients and operators}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash C\#1 \textbackslash C9} & \C9 & \texttt{\textbackslash Cp\#1 \textbackslash Cp7} & \Cp7 & \texttt{\textbackslash Ceff\#1 \textbackslash Ceff9  } & \Ceff9   \\
\texttt{\textbackslash Cpeff\#1 \textbackslash Cpeff7} & \Cpeff7 & \texttt{\textbackslash Ope\#1 \textbackslash Ope2} & \Ope2 & \texttt{\textbackslash Opep\#1 \textbackslash Opep7} & \Opep7 \\
\end{tabular*}

\subsubsection{Charm}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash xprime} & \xprime & \texttt{\textbackslash yprime} & \yprime & \texttt{\textbackslash ycp} & \ycp \\
\texttt{\textbackslash agamma} & \agamma & \texttt{\textbackslash dkpicf} & \dkpicf &  \\
\end{tabular*}

\subsubsection{QM}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bra[1] \textbackslash bra\{a\}} & \bra{a} & \texttt{\textbackslash ket[1] \textbackslash ket\{b\}} & \ket{b} & \texttt{\textbackslash braket[2] \textbackslash braket\{a\}\{b\}} & \braket{a}{b} \\
\end{tabular*}

\subsection{Units}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash unit[1] \textbackslash unit\{kg\}} & \unit{kg} &  \\
\end{tabular*}

\subsubsection{Energy and momentum}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tev} & \tev & \texttt{\textbackslash gev} & \gev & \texttt{\textbackslash mev} & \mev \\
\texttt{\textbackslash kev} & \kev & \texttt{\textbackslash ev} & \ev & \texttt{\textbackslash gevc} & \gevc \\
\texttt{\textbackslash mevc} & \mevc & \texttt{\textbackslash gevcc} & \gevcc & \texttt{\textbackslash gevgevcccc} & \gevgevcccc \\
\texttt{\textbackslash mevcc} & \mevcc &  \\
\end{tabular*}

\subsubsection{Distance and area}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash km} & \km & \texttt{\textbackslash m} & \m & \texttt{\textbackslash ma} & \ma \\
\texttt{\textbackslash cm} & \cm & \texttt{\textbackslash cma} & \cma & \texttt{\textbackslash mm} & \mm \\
\texttt{\textbackslash mma} & \mma & \texttt{\textbackslash mum} & \mum & \texttt{\textbackslash muma} & \muma \\
\texttt{\textbackslash nm} & \nm & \texttt{\textbackslash fm} & \fm & \texttt{\textbackslash barn} & \barn \\
\texttt{\textbackslash mbarn} & \mbarn & \texttt{\textbackslash mub} & \mub & \texttt{\textbackslash nb} & \nb \\
\texttt{\textbackslash invnb} & \invnb & \texttt{\textbackslash pb} & \pb & \texttt{\textbackslash invpb} & \invpb \\
\texttt{\textbackslash fb} & \fb & \texttt{\textbackslash invfb} & \invfb & \texttt{\textbackslash ab} & \ab \\
\texttt{\textbackslash invab} & \invab &  \\
\end{tabular*}

\subsubsection{Time }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sec} & \sec & \texttt{\textbackslash ms} & \ms & \texttt{\textbackslash mus} & \mus \\
\texttt{\textbackslash ns} & \ns & \texttt{\textbackslash ps} & \ps & \texttt{\textbackslash fs} & \fs \\
\texttt{\textbackslash mhz} & \mhz & \texttt{\textbackslash khz} & \khz & \texttt{\textbackslash hz} & \hz \\
\texttt{\textbackslash invps} & \invps & \texttt{\textbackslash invns} & \invns & \texttt{\textbackslash yr} & \yr \\
\texttt{\textbackslash hr} & \hr &  \\
\end{tabular*}

\subsubsection{Temperature}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degc} & \degc & \texttt{\textbackslash degk} & \degk &  \\
\end{tabular*}

\subsubsection{Material lengths, radiation}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Xrad} & \Xrad & \texttt{\textbackslash NIL} & \NIL & \texttt{\textbackslash mip} & \mip \\
\texttt{\textbackslash neutroneq} & \neutroneq & \texttt{\textbackslash neqcmcm} & \neqcmcm & \texttt{\textbackslash kRad} & \kRad \\
\texttt{\textbackslash MRad} & \MRad & \texttt{\textbackslash ci} & \ci & \texttt{\textbackslash mci} & \mci \\
\end{tabular*}

\subsubsection{Uncertainties}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash sx} & \sx & \texttt{\textbackslash sy} & \sy & \texttt{\textbackslash sz} & \sz \\
\texttt{\textbackslash stat} & \stat & \texttt{\textbackslash syst} & \syst &  \\
\end{tabular*}

\subsubsection{Maths}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash order} & \order & \texttt{\textbackslash chisq} & \chisq & \texttt{\textbackslash chisqndf} & \chisqndf \\
\texttt{\textbackslash chisqip} & \chisqip & \texttt{\textbackslash chisqvs} & \chisqvs & \texttt{\textbackslash chisqvtx} & \chisqvtx \\
\texttt{\textbackslash chisqvtxndf} & \chisqvtxndf & \texttt{\textbackslash deriv} & \deriv & \texttt{\textbackslash gsim} & \gsim \\
\texttt{\textbackslash lsim} & \lsim & \texttt{\textbackslash mean[1] \textbackslash mean\{x\}} & \mean{x} & \texttt{\textbackslash abs[1] \textbackslash abs\{x\}} & \abs{x} \\
\texttt{\textbackslash Real} & \Real & \texttt{\textbackslash Imag} & \Imag & \texttt{\textbackslash PDF} & \PDF \\
\texttt{\textbackslash sPlot} & \sPlot &  \\
\end{tabular*}

\subsection{Kinematics}
\subsubsection{Energy, Momenta}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash Ebeam} & \Ebeam & \texttt{\textbackslash sqs} & \sqs & \texttt{\textbackslash ptot} & \ptot \\
\texttt{\textbackslash pt} & \pt & \texttt{\textbackslash et} & \et & \texttt{\textbackslash mt} & \mt \\
\texttt{\textbackslash dpp} & \dpp & \texttt{\textbackslash msq} & \msq & \texttt{\textbackslash dedx} & \dedx \\
\end{tabular*}

\subsubsection{PID}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash dllkpi} & \dllkpi & \texttt{\textbackslash dllppi} & \dllppi & \texttt{\textbackslash dllepi} & \dllepi \\
\texttt{\textbackslash dllmupi} & \dllmupi &  \\
\end{tabular*}

\subsubsection{Geometry}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash degrees} & \degrees & \texttt{\textbackslash krad} & \krad & \texttt{\textbackslash mrad} & \mrad \\
\texttt{\textbackslash rad} & \rad &  \\
\end{tabular*}

\subsubsection{Accelerator}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash betastar} & \betastar & \texttt{\textbackslash lum} & \lum & \texttt{\textbackslash intlum[1] \textbackslash intlum\{2 \,\invfb\}} & \intlum{2 \,\invfb} \\
\end{tabular*}

\subsection{Software}
\subsubsection{Programs}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash bcvegpy} & \bcvegpy & \texttt{\textbackslash boole} & \boole & \texttt{\textbackslash brunel} & \brunel \\
\texttt{\textbackslash davinci} & \davinci & \texttt{\textbackslash dirac} & \dirac & \texttt{\textbackslash evtgen} & \evtgen \\
\texttt{\textbackslash fewz} & \fewz & \texttt{\textbackslash fluka} & \fluka & \texttt{\textbackslash ganga} & \ganga \\
\texttt{\textbackslash gaudi} & \gaudi & \texttt{\textbackslash gauss} & \gauss & \texttt{\textbackslash geant} & \geant \\
\texttt{\textbackslash hepmc} & \hepmc & \texttt{\textbackslash herwig} & \herwig & \texttt{\textbackslash moore} & \moore \\
\texttt{\textbackslash neurobayes} & \neurobayes & \texttt{\textbackslash photos} & \photos & \texttt{\textbackslash powheg} & \powheg \\
\texttt{\textbackslash pythia} & \pythia & \texttt{\textbackslash resbos} & \resbos & \texttt{\textbackslash roofit} & \roofit \\
\texttt{\textbackslash root} & \root & \texttt{\textbackslash spice} & \spice & \texttt{\textbackslash urania} & \urania \\
\end{tabular*}

\subsubsection{Languages}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cpp} & \cpp & \texttt{\textbackslash ruby} & \ruby & \texttt{\textbackslash fortran} & \fortran \\
\texttt{\textbackslash svn} & \svn &  \\
\end{tabular*}

\subsubsection{Data processing}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash kbytes} & \kbytes & \texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash kbits} & \kbits \\
\texttt{\textbackslash kbsps} & \kbsps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash mbytes} & \mbytes \\
\texttt{\textbackslash mbps} & \mbps & \texttt{\textbackslash mbsps} & \mbsps & \texttt{\textbackslash gbsps} & \gbsps \\
\texttt{\textbackslash gbytes} & \gbytes & \texttt{\textbackslash gbsps} & \gbsps & \texttt{\textbackslash tbytes} & \tbytes \\
\texttt{\textbackslash tbpy} & \tbpy & \texttt{\textbackslash dst} & \dst &  \\
\end{tabular*}

\subsection{Detector related}
\subsubsection{Detector technologies}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash nonn} & \nonn & \texttt{\textbackslash ponn} & \ponn & \texttt{\textbackslash nonp} & \nonp \\
\texttt{\textbackslash cvd} & \cvd & \texttt{\textbackslash mwpc} & \mwpc & \texttt{\textbackslash gem} & \gem \\
\end{tabular*}

\subsubsection{Detector components, electronics}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash tell1} & \tell1 & \texttt{\textbackslash ukl1} & \ukl1 & \texttt{\textbackslash beetle} & \beetle \\
\texttt{\textbackslash otis} & \otis & \texttt{\textbackslash croc} & \croc & \texttt{\textbackslash carioca} & \carioca \\
\texttt{\textbackslash dialog} & \dialog & \texttt{\textbackslash sync} & \sync & \texttt{\textbackslash cardiac} & \cardiac \\
\texttt{\textbackslash gol} & \gol & \texttt{\textbackslash vcsel} & \vcsel & \texttt{\textbackslash ttc} & \ttc \\
\texttt{\textbackslash ttcrx} & \ttcrx & \texttt{\textbackslash hpd} & \hpd & \texttt{\textbackslash pmt} & \pmt \\
\texttt{\textbackslash specs} & \specs & \texttt{\textbackslash elmb} & \elmb & \texttt{\textbackslash fpga} & \fpga \\
\texttt{\textbackslash plc} & \plc & \texttt{\textbackslash rasnik} & \rasnik & \texttt{\textbackslash elmb} & \elmb \\
\texttt{\textbackslash can} & \can & \texttt{\textbackslash lvds} & \lvds & \texttt{\textbackslash ntc} & \ntc \\
\texttt{\textbackslash adc} & \adc & \texttt{\textbackslash led} & \led & \texttt{\textbackslash ccd} & \ccd \\
\texttt{\textbackslash hv} & \hv & \texttt{\textbackslash lv} & \lv & \texttt{\textbackslash pvss} & \pvss \\
\texttt{\textbackslash cmos} & \cmos & \texttt{\textbackslash fifo} & \fifo & \texttt{\textbackslash ccpc} & \ccpc \\
\end{tabular*}

\subsubsection{Chemical symbols}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash cfourften} & \cfourften & \texttt{\textbackslash cffour} & \cffour & \texttt{\textbackslash cotwo} & \cotwo \\
\texttt{\textbackslash csixffouteen} & \csixffouteen & \texttt{\textbackslash mgftwo} & \mgftwo & \texttt{\textbackslash siotwo} & \siotwo \\
\end{tabular*}

\subsection{Special Text }
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}
\texttt{\textbackslash eg} & \eg & \texttt{\textbackslash ie} & \ie & \texttt{\textbackslash etal} & \etal \\
\texttt{\textbackslash etc} & \etc & \texttt{\textbackslash cf} & \cf & \texttt{\textbackslash ffp} & \ffp \\
\texttt{\textbackslash vs} & \vs &  \\
\end{tabular*}



==> principles.tex <==
\section{General principles}

The main goal is for a paper to be clear. It should be as brief as
possible, without sacrificing clarity. For all public documents,
special consideration should be given to the fact that the reader will
be less familiar with \lhcb than the author.

Here follow a list of general principles that should be adhered to:
\begin{enumerate}

\item Choices that are made concerning layout and typography
  should be consistently applied throughout the document.

\item Standard English should be used (British rather than American)
  for LHCb notes and preprints. Examples: colour, flavour, centre,
  metre, modelled and aluminium. Words ending on -ise or -isation
  (polarise, hadronisation) can be written with -ize or -ization ending.
  The punctuation normally follows the closing
  quote mark of quoted text, rather than being included before the
  closing quote.
  Footnotes come after punctuation. 
  Papers to be submitted to an American journal can be written in American
  English instead. Under no circumstance should the two be mixed.

\item Use of jargon should be avoided where possible. ``Systematics'' are ``systematic
  uncertainties'', ``L0'' is ``hardware trigger'', ``penguin'' diagrams
  are best introduced with an expression like ``electroweak loop (penguin) diagrams''.

\item Avoid using quantities that are internal jargon and/or are impossible to reproduce without the full simulation:
instead of `It is required that $\chisqvtx<3$', say 'A good quality vertex is required';
instead of `It is required that $\chisqip>16$', say `The track is inconsistent with originating from a PV';
instead of `A DLL greater than 20 is required' say `Tracks are required to be identified as kaons'.


\item Latex should be used for typesetting. Line numbering should be
  switched on for drafts that are circulated for comments.

\item The abstract should be concise, and not include citations or
  numbered equations, and should give the key results from the paper.

\item Apart from descriptions of the detector, the trigger and the
  simulation, the text should not be cut-and-pasted from other sources
  that have previously been published.

\item References should usually be made only to publicly accessible
  documents. References to LHCb conference reports and public notes
  should be avoided in journal publications, instead including the
  relevant material in the paper itself.

\item The use of tenses should be consistent. It is recommended to
  mainly stay in the present tense, for the abstract, the description
  of the analysis, \etc; the past tense is then used where necessary,
  for example when describing the data taking conditions.

\item It is recommended to use the passive rather than active voice:
  ``the mass is measured'', rather than ``we measure the mass''.
  Limited use of the active voice is acceptable, in situations where
  re-writing in the passive form would be cumbersome, such as for the
  acknowledgements.  Some leeway is permitted to accommodate different
  author's styles, but ``we'' should not appear excessively in the
  abstract or the first lines of introduction or conclusion.

\item A sentence should not start with a variable, a particle or an acronym. A title or caption should not start with an article. 

\item Incorrect punctuation around conjunctive adverbs and the use of 
dangling modifiers are the two most common mistakes of English grammar
in LHCb draft papers. If in doubt, read the wikipedia articles on 
conjunctive adverb and dangling modifier.  

\end{enumerate}


==> reference.tex <==
\section{References}
\label{sec:References}

References should be made using Bib\TeX~\cite{BibTeX}. A special style
\texttt{LHCb.bst} has been created to achieve a uniform
style. Independent of the journal the paper is submitted to, the
preprint should be created using this style. Where arXiv numbers
exist, these should be added even for published articles. In the PDF
file, hyperlinks will be created to both the arXiv and the published
version.

\begin{enumerate}

\item Citations are marked using square brackets, and the
  corresponding references should be typeset using Bib\TeX\ and the
  official \lhcb Bib\TeX\ style. An example is in
  Ref.~\cite{Sjostrand:2006za}.

\item For references with four or less authors all of the authors'
  names are listed~\cite{Majorana:1937vz}, otherwise the first author
  is given, followed by \etal. The \lhcb Bib\TeX\ style will
  take care of this.

\item The order of references should be sequential when reading the
  document. This is automatic when using Bib\TeX.

\item The titles of papers should in general be included. To remove
  them, change \texttt{\textbackslash
    setboolean\{articletitles\}\{false\}} to \texttt{true} at the top
  of this template.
  Note that the titles in \verb!LHCb-PAPER.bib! are in plain LaTex,
  in order to correspond to the actual title on the arXiv record.
  Some differences in style can thus be noticed with respect to the
  main text, for example particle names that use capital Greek letters
  are not slanted in the reference titles ($\Lambda$ vs \Lz)  

\item Whenever possible, use references from the supplied files
\verb!main.bib!, \verb!LHCb-PAPER.bib!, \verb!LHCb-CONF.bib!, and \verb!LHCB-DP.bib!.
These are kept up-to-date by the EB. If you see a mistake, do not edit these files,
but let the EB know. This way, for every update of the paper, you save
yourself the work of updating the references. Instead, you can just copy or
check in the latest versions of the \verb!.bib! files from the repository.   

\item For those references not provided by the EB, the best
  is to copy the Bib\TeX\ entry directly from
  \texttt{Inspire}. Often these need to be edited to get the 
  correct title, author names and formatting.
  For authors with multiple initials, add a space between them (change \texttt{R.G.C.} to \texttt{R. G. C.}),
  otherwise only the first initial will be taken. 
  Also, make sure to eliminate unnecessary capitalisation.
  Apart from that, the title should be respected as much as possible
  (\eg do not change particle names to PDG convention nor introduce/remove factors of $c$).
  Check that both the arXiv and the journal index are clickable
  and point to the right article.

%\item Even if the basic formatting of the Bib\TeX\ entry is taken from
%  \texttt{Inspire}, all the data should be cross checked against the
%  journal. Often there are minor changes to author initials or
%  titles. In case of a difference between the preprint and the
%  journal, the bibliographic information from the journal should be
%  used.

\item The \texttt{mciteplus}~\cite{mciteplus} package is used
  to enable multiple references to show up as a single item in the
  reference list. As an example \texttt{\textbackslash
    cite\{Mohapatra:1979ia,*Pascoli:2007qh\}} where the \texttt{*}
  indicates that the reference should be merged with the previous
  one. The result of this can be seen in
  Ref.~\cite{Mohapatra:1979ia,*Pascoli:2007qh}. Be aware that the
  \texttt{mciteplus} package should be included as the very last item
  before the \texttt{\textbackslash begin\{document\}} to work
  correctly.

\item It should be avoided to make references to public notes and
  conference reports in public documents. Exceptions can be discussed
  on a case-by-case basis with the review committee for the
  analysis. In internal reports they are of course welcome and can be
  referenced as seen in Ref.~\cite{LHCb-CONF-2011-003} using the
  \texttt{lhcbreport} category. For conference reports, omit the
  author field completely in the Bib\TeX\ record.

\item To get the typesetting and hyperlinks correct for \lhcb reports,
  the category \texttt{lhcbreport} should be used in the Bib\TeX\
  file. See Refs.~\cite{LHCb-INT-2011-047, *LHCb-ANA-2011-078,
    *CERN-THESIS-2014-057, *LHCb-PROC-2014-017, *LHCB-TALK-2014-257}
  for some examples. It can be used for \lhcb documents in the series
  \texttt{CONF}, \texttt{PAPER}, \texttt{PROC}, \texttt{THESIS},
  \texttt{LHCC}, \texttt{TDR} and internal \lhcb reports. Papers sent
  for publication, but not published yet, should be referred with
  their \texttt{arXiv} number, so the \texttt{PAPER} category should
  only be used in the rare case of a forward reference to a paper.

\item Proceedings can be used for references to items such as the
  \lhcb simulation~\cite{LHCb-PROC-2011-006}, where we do not yet have
  a published paper.

\end{enumerate}

There is a set of standard references to be used in \lhcb that are
listed in Appendix~\ref{sec:StandardReferences}.


==> title-LHCb-ANA.tex <==
% $Id: title-LHCb-ANA.tex 39841 2013-07-26 10:31:08Z roldeman $
% ===============================================================================
% Purpose: LHCb-ANA Note title page template
% Author: 
% Created on: 2010-10-05
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}

% Header ---------------------------------------------------
\vspace*{-1.5cm}

\noindent
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r@{\extracolsep{0pt}}}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-2.7cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{lhcb-logo.eps}} & &}
 \\
 & & LHCb-ANA-20XX-YYY \\  % ID 
 & & \today \\ % Date - Can also hardwire e.g.: 23 March 2010
 & & \\
\hline
\end{tabular*}

\vspace*{4.0cm}

% Title --------------------------------------------------
{\normalfont\bfseries\boldmath\huge
\begin{center}
  A template for writing LHCb documents
\end{center}
}

\vspace*{2.0cm}

% Authors -------------------------------------------------
\begin{center}
U.~Egede$^1$.
\bigskip\\
{\normalfont\itshape\footnotesize
$ ^1$Imperial College London, London, United Kingdom\\
}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
  Guidelines for the preparation of LHCb documents are given. This is
  a ``living'' document, that should reflect our current practice. It
  is expected that these guidelines are implemented for papers already
  before they go into the first collaboration wide review. Please
  contact the Editorial Board chair if you have suggestions for
  modifications.
\end{abstract}

\vspace*{2.0cm}
\vspace{\fill}

\end{titlepage}


\pagestyle{empty}  % no page number for the title 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}

\cleardoublepage


==> title-LHCb-CONF.tex <==
% $Id: title-LHCb-CONF.tex 28385 2012-11-23 17:37:51Z uegede $
% ===============================================================================
% Purpose: LHCb-CONF Note title page template
% Author:
% Created on: 2010-09-25
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}

% Header ---------------------------------------------------
\vspace*{-1.5cm}

\hspace*{-0.5cm}
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{figs/lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{figs/lhcb-logo.eps}} & &}
 \\
 & & LHCb-CONF-2016-001 \\  % ID
 & & \today \\ % Date - Can also hardwire e.g.: 23 March 2010
 %& & version 7\\
\hline
\end{tabular*}

\vspace*{4.0cm}

% Title --------------------------------------------------
{\bf\boldmath\huge
\begin{center}
Measurement of the CKM angle $\gamma$ from a combination of $B\to DK$ analyses
%  LHCb $\gamma$ combination using $B \to DK$ decays
%  \\ Rencontres de Moriond 2016 update
\end{center}
}

\vspace*{1.5cm}

% Authors -------------------------------------------------
\begin{center}
The LHCb collaboration
% Identify conference in the footnote
\footnote{Conference report prepared for the Rencontres de Moriond
	Electroweak, $12^{\rm th}$--$19^{\rm th}$ March 2016, La Thuile.
		Contact authors:
Matthew Kenzie (\href{mailto:matthew.william.kenzie@cern.ch}{matthew.william.kenzie@cern.ch}),
Mark Whitehead (\href{mailto:mark.peter.whitehead@cern.ch}{mark.peter.whitehead@cern.ch}).
}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
\noindent
A combination is made of tree-level measurements of the CKM angle $\gamma$ from $B \to DK$ decays
at \lhcb. The results are obtained from time-integrated
analyses of \BuDK, \BdDKstz and \BuDKpipi decays,
where the $D$ meson decays into \KK, \pipi, \KKpiz, \Kpipiz, \pipipiz, \Kpi, \KSKpi, \KSpipi, \KSKK,
\Kpipipi and \pipipipi final states.
%The effect of \Dz--\Dzb mixing is taken into account.
In addition, results obtained from a time-dependent
analysis of \BsDsK decays are included.
The combination gives a best fit value of $\g = \gRobustCentral^\circ$ and
confidence intervals are set using a frequentist procedure:
$\g \in \gRobustOnesig^\circ$ at 68\% CL and
$\g \in \gRobustTwosig^\circ$ at 95\% CL,
where all values are modulo $180^\circ$.
Using the best fit value and the 68\% CL interval, $\gamma$ is measured to be
\begin{align*}
\g = (\gQuoted)^\circ\,,
\end{align*}
where the quoted uncertainty is the statistical and systematic combined.
This is the most precise single-experiment measurement of the CKM angle $\gamma$ to date.
\end{abstract}

\vspace*{0.5cm}
\vspace{\fill}
{\footnotesize
\centerline{\copyright~CERN on behalf of the \lhcb collaboration, license \href{http://creativecommons.org/licenses/by/4.0/}{CC-BY-4.0}.}}
\vspace*{2mm}

\end{titlepage}

\pagestyle{empty}  % no page number for the title

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}

\cleardoublepage


==> title-LHCb-INT.tex <==
% $Id: title-LHCb-INT.tex  $
% ===============================================================================
% Purpose: LHCb-INT Note title page template
% Author: P. Koppenburg
% Created on: 2015-05-18
% ===============================================================================

%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{titlepage}

% Header ---------------------------------------------------
\vspace*{-1.5cm}

\noindent
\begin{tabular*}{\linewidth}{lc@{\extracolsep{\fill}}r@{\extracolsep{0pt}}}
\ifthenelse{\boolean{pdflatex}}% Logo format choice
{\vspace*{-2.7cm}\mbox{\!\!\!\includegraphics[width=.14\textwidth]{lhcb-logo.pdf}} & &}%
{\vspace*{-1.2cm}\mbox{\!\!\!\includegraphics[width=.12\textwidth]{lhcb-logo.eps}} & &}
 \\
 & & LHCb-INT-20XX-YYY \\  % ID 
 & & \today \\ % Date - Can also hardwire e.g.: 23 March 2010
 & & \\
\hline
\end{tabular*}

\vspace*{4.0cm}

% Title --------------------------------------------------
{\normalfont\bfseries\boldmath\huge
\begin{center}
  A template for writing LHCb documents
\end{center}
}

\vspace*{2.0cm}

% Authors -------------------------------------------------
\begin{center}
U.~Egede$^1$.
\bigskip\\
{\normalfont\itshape\footnotesize
$ ^1$Imperial College London, London, United Kingdom\\
}
\end{center}

\vspace{\fill}

% Abstract -----------------------------------------------
\begin{abstract}
  \noindent
  Guidelines for the preparation of LHCb documents are given. This is
  a ``living'' document, that should reflect our current practice. It
  is expected that these guidelines are implemented for papers already
  before they go into the first collaboration wide review. Please
  contact the Editorial Board chair if you have suggestions for
  modifications.
\end{abstract}

\vspace*{2.0cm}
\vspace{\fill}

\end{titlepage}


\pagestyle{empty}  % no page number for the title 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%  EOD OF TITLE PAGE  %%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%  empty page follows the title page ----
\newpage
\setcounter{page}{2}
\mbox{~}

\cleardoublepage


==> typography.tex <==
\section{Typography}
\label{sec:typography}

The use of the Latex typesetting symbols defined in the file
\texttt{lhcb-symbols-def.tex} and detailed in the appendices of this
document is strongly encouraged as it will make it much easier to
follow the recommendation set out below.

\begin{enumerate}

\item \lhcb is typeset with a normal (roman) lowercase b.

\item Titles are in bold face, and usually only the first word is
  capitalised.

\item Mathematical symbols and particle names should also be typeset
  in bold when appearing in titles.

\item Units are in roman type, except for constants such as $c$ or $h$
  that are italic: \gev, \gevcc.  The unit should be separated from
  the value with a thin space (``\verb!\,!''),
  and they should not be broken over two lines.
  Correct spacing is automatic when using predefined units inside math mode: \verb!$3.0\gev$! $\to 3.0\gev$.
  Spacing goes wrong when using predefined units outside math mode AND forcing extra space:
  \verb!3.0\,\gev! $\to$ 3.0\,\gev or worse:   \verb!3.0~\gev! $\to$ 3.0~\gev. 

\item  If factors of $c$ are kept, they should be used both for masses and
  momenta, \eg $p=5.2\gevc$ (or $\gev c^{-1}$), $m = 3.1\gevcc$ (or $\gev c^{-2}$). If they are dropped this
  should be done consistently throughout, and a note should be added
  at the first instance to indicate that units are taken with $c=1$.

\item The \% sign should not be separated from the number that precedes it: 5\%, not 5 \%. 
A thin space is also acceptable: 5\,\%, but should be applied consistently throughout the paper.

\item Ranges should be formatted consistently. The recommendend form is to use a dash with no spacing around it: 
7--8\gev, obtained as \verb!7--8\gev!. 

\item Italic is preferred for particle names (although roman is
  acceptable, if applied consistently throughout).  Particle Data
  Group conventions should generally be followed: \Bd (no need for a
  ``d'' subscript), \decay{\Bs}{\jpsi\phi}, \Bsb,
  (note the long bar, obtained with \verb!\overline!, in contrast to the discouraged short \verb!\bar{B}! resulting in $\bar{B}$), \KS (note the
  uppercase roman type ``S''). 
This is most easily achieved by using the predefined symbols described in 
  Appendix~\ref{sec:listofsymbols}.
  Unless there is a good reason not to, the charge of a particle should be
  specified if there is any possible ambiguity 
  ($m(\Kp\Km)$ instead of $m(KK)$, which could refer to neutral kaons).

\item Decay chains can be written in several ways, depending on the complexity and the number of times it occurs. Unless there is a good reason not to, usage of a particular type should be consistent within the paper.
Examples are: 
$\Dsp\to\phi\pip$, with $\phi\to\Kp\Km$; 
$\Dsp\to\phi\pip$ ($\phi\to\Kp\Km$);  
$\Dsp\to\phi(\to\Kp\Km)\pip$; or
$\Dsp\to[\Kp\Km]_\phi\pip$.



\item Variables are usually italic: $V$ is a voltage (variable), while
  1 V is a volt (unit). Also in combined expressions: $Q$-value, $z$-scale, $R$-parity \etc

\item Subscripts and superscripts are roman type when they refer to a word (such as T
  for transverse) and italic when they refer to a variable (such as
  $t$ for time): \pt, \dms, $t_{\mathrm{rec}}$.

\item Standard function names are in roman type: \eg $\cos$, $\sin$
  and $\exp$.

\item Figure, Section, Equation, Chapter and Reference should be
  abbreviated as Fig., Sect. (or alternatively Sec.), Eq., Chap.\ and
  Ref.\ respectively, when they refer to a particular (numbered) item,
  except when they start a sentence. Table and Appendix are not
  abbreviated.  The plural form of abbreviation keeps the point after
  the s, \eg Figs.~1 and~2. Equations may be referred to either with 
  (``Eq.~(1)'') or without (``Eq.~1'') parentheses, 
  but it should be consistent within the paper.

\item Common abbreviations derived from Latin such as ``for example''
  (\eg), ``in other words'' (\ie), ``and so forth'' (\etc), ``and
  others'' (\etal), ``versus'' (\vs) can be used, with the typography
  shown, but not excessively; other more esoteric abbreviations should be avoided.
  

\item Units, material and particle names are usually lower case if
  spelled out, but often capitalised if abbreviated: amps (A), gauss
  (G), lead (Pb), silicon (Si), kaon (\kaon), but proton (\proton).

%\item The prefix for 1000 (k, \eg kV) should not be confused with
%  that used in computing (K, which strictly speaking denotes $2^{10}$,
%  \eg KB).

\item Counting numbers are usually written in words if they start a
  sentence or if they have a value of ten or below in descriptive
  text (\ie not including figure numbers such as ``Fig.\ 4'', or
  values followed by a unit such as ``4\,cm'').
  The word 'unity' can be useful to express the special meaning of
  the number one in expressions such as: 
``The BDT output takes values between zero and unity''.
% Numbers should not be
%  written as words if they by nature are real numbers that happen to
%  take an integer value, such as $\chisq/\mathrm{ndf} < 4$.

\item Numbers larger than 9999 have a comma (or a small space, but not both) between
  the multiples of thousand: \eg 10,000 or 12,345,678.  The decimal
  point is indicated with a point rather than a comma: \eg 3.141.

\item We apply the rounding rules of the
  PDG~\cite{PDG2014}. The basic rule states that if the three
  highest order digits of the uncertainty lie between 100 and 354, we round
  to two significant digits. If they lie between 355 and 949, we round
  to one significant digit. Finally, if they lie between 950 and 999,
  we round up and keep two significant digits. In all cases,
  the central value is given with a precision that matches that of the
  uncertainty. So, for example, the result $0.827 \pm 0.119$ should be
  written as $0.83\pm 0.12$, $0.827\pm 0.367$ should turn into
  $0.8\pm 0.4$, and $14.674\pm0.964$ becomes $14.7\pm1.0$.
 When writing numbers with uncertainty components from
  different sources, \ie statistical and systematic uncertainties, the rule
  applies to the uncertainty with the best precision, so $0.827\pm
  0.367\stat\pm 0.179\syst$ goes to $0.83\pm 0.37\stat\pm 0.18\syst$ and
  $8.943\pm 0.123\stat\pm 0.995\syst$ goes to $8.94\pm 0.12\stat\pm
  1.00\syst$.

\item When rounding numbers, it should be avoided to pad with zeroes
  at the end. So $51237 \pm 4561$ should be rounded as $(5.12 \pm 0.46)
  \times 10^4$ and not $51200 \pm 4600$.

\item When rounding numbers in a table, some variation of the rounding
  rules above may be required to achieve uniformity.

\item Hyphenation should be used where necessary to avoid ambiguity,
  but not excessively. For example: ``big-toothed fish''
  (to indicate that big refers to the teeth, not to the fish),
  but ``big white fish''.
  A compound modifier often requires hyphenation 
  (\CP-violating observables, \bquark-hadron decays, final-state radiation, second-order polynomial),
  even if the same combination in an adjective-noun combination does not
  (direct \CP violation, heavy \bquark hadrons, charmless final state).
  Adverb-adjective combinations are not hyphenated if the adverb ends with 'ly':
  oppositely charged pions, kinematically similar decay.
  Cross-section, cross-check, and two-dimensional are hyphenated.
  Semileptonic, pseudorapidity, pseudoexperiment, multivariate, multidimensional, reweighted, preselection, 
  nonresonant, nonzero, nonparametric, nonrelativistic, misreconstructed and misidentified
  are single words and should not be hyphenated.

\item Minus signs should be in a proper font ($-1$), not just hyphens
  (-1); this applies to figure labels as well as the body of the text.
  In Latex, use math mode (between \verb!$$!'s) or make a dash (``\verb!--!'').
  In ROOT, use \verb!#font[122]{-}! to get a normal-sized minus sign. 

\item Inverted commas (around a title, for example) should be a
  matching set of left- and right-handed pairs: ``Title''. The use of
  these should be avoided where possible.

\item Single symbols are preferred for variables in equations, \eg\
  \BF\ rather than BF for a branching fraction.

\item Parentheses are not usually required around a value and its
  uncertainty, before the unit, unless there is possible ambiguity: so
  $\dms = 20 \pm 2\invps$ does not need parentheses, whereas $f_d =
  (40 \pm 4)$\% or $x=(1.7\pm0.3)\times 10^{-6}$ does.
  The unit does not need to be repeated in
  expressions like $1.2 < E < 2.4\gev$.

\item The same number of decimal places should be given for all values
  in any one expression (\eg $5.20 < m_B < 5.34\gevcc$).

\item Apostrophes are best avoided for abbreviations: if the abbreviated term
  is capitalised or otherwise easily identified then the plural can simply add
  an s, otherwise it is best to rephrase: \eg HPDs, \pizs, pions, rather
  than HPD's, \piz's, $\pion$s.

\item Particle labels, decay descriptors and mathematical functions are not nouns, and need often to be followed by a noun. 
Thus ``background from $\Bd\to\pi^+\pi^-$ decays'' instead of ``background from $\Bd\to\pi^+\pi^-$'',
and ``the width of the Gaussian function'' instead of ``the width of the Gaussian''.

\item In equations with multidimensional integrations or differentiations, the differential terms should be separated by a thin space. 
Thus $\int f(x,y) dx\,dy$ instead $\int f(x,y) dxdy$ and
$\frac{d^2\Gamma}{dx\,dQ^2}$ instead of $\frac{d^2\Gamma}{dxdQ^2}$.
The d's are allowed in either roman or italic font, but should be consistent throughout the paper.


\end{enumerate}


==> validation.tex <==
%\clearpage

\section{Cross checks}
\label{sec:validation}

Cross checks of the statistical procedure are summarised in this section which documents
the coverage of the frequentist method in Sec.~\ref{sec:coverage} and the results of
a Bayesian implementation in Sec.~\ref{sec:bayesian}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa

